All-optical source size and emittance measurements of laser-accelerated electron beams

Novel schemes for generating ultra-low emittance electron beams have been developed in past years and promise compact particle sources with excellent beam quality suitable for future high-energy physics experiments and free-electron lasers. Recent theoretical work has proposed a laser-based method capable of resolving emittances in the sub 0.1 mm mrad regime, by modulating the electron phase-space ponderomotively. Here we present a first experimental demonstration of this scheme using a laser wakefield accelerator. The observed emittance and source size is consistent with published values. We also show calculations demonstrating that tight bounds on the upper limit for emittance and source size can be derived from the 'laser-grating' method even in the presence of low signal to noise and uncertainty in laser-grating parameters.

==> references.tex <==
\begin{thebibliography}{55}%
\makeatletter
\providecommand \@ifxundefined [1]{%
 \@ifx{#1\undefined}
}%
\providecommand \@ifnum [1]{%
 \ifnum #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \@ifx [1]{%
 \ifx #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \natexlab [1]{#1}%
\providecommand \enquote  [1]{``#1''}%
\providecommand \bibnamefont  [1]{#1}%
\providecommand \bibfnamefont [1]{#1}%
\providecommand \citenamefont [1]{#1}%
\providecommand \href@noop [0]{\@secondoftwo}%
\providecommand \href [0]{\begingroup \@sanitize@url \@href}%
\providecommand \@href[1]{\@@startlink{#1}\@@href}%
\providecommand \@@href[1]{\endgroup#1\@@endlink}%
\providecommand \@sanitize@url [0]{\catcode `\\12\catcode `\$12\catcode
  `\&12\catcode `\#12\catcode `\^12\catcode `\_12\catcode `\%12\relax}%
\providecommand \@@startlink[1]{}%
\providecommand \@@endlink[0]{}%
\providecommand \url  [0]{\begingroup\@sanitize@url \@url }%
\providecommand \@url [1]{\endgroup\@href {#1}{\urlprefix }}%
\providecommand \urlprefix  [0]{URL }%
\providecommand \Eprint [0]{\href }%
\providecommand \doibase [0]{https://doi.org/}%
\providecommand \selectlanguage [0]{\@gobble}%
\providecommand \bibinfo  [0]{\@secondoftwo}%
\providecommand \bibfield  [0]{\@secondoftwo}%
\providecommand \translation [1]{[#1]}%
\providecommand \BibitemOpen [0]{}%
\providecommand \bibitemStop [0]{}%
\providecommand \bibitemNoStop [0]{.\EOS\space}%
\providecommand \EOS [0]{\spacefactor3000\relax}%
\providecommand \BibitemShut  [1]{\csname bibitem#1\endcsname}%
\let\auto@bib@innerbib\@empty
\bibitem [{\citenamefont {Esarey}\ \emph {et~al.}(2009)\citenamefont {Esarey},
  \citenamefont {Schroeder},\ and\ \citenamefont {Leemans}}]{Esarey.2009}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Esarey}}, \bibinfo {author} {\bibfnamefont {C.~B.}\ \bibnamefont
  {Schroeder}},\ and\ \bibinfo {author} {\bibfnamefont {W.~P.}\ \bibnamefont
  {Leemans}},\ }\bibfield  {title} {\bibinfo {title} {{Physics of laser-driven
  plasma-based electron accelerators}},\ }\href
  {https://doi.org/10.1103/RevModPhys.81.1229} {\bibfield  {journal} {\bibinfo
  {journal} {Rev. Mod. Phys.}\ }\textbf {\bibinfo {volume} {81}},\ \bibinfo
  {pages} {1229} (\bibinfo {year} {2009})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Gonsalves}\ \emph {et~al.}(2019)\citenamefont
  {Gonsalves}, \citenamefont {Nakamura}, \citenamefont {Daniels}, \citenamefont
  {Benedetti}, \citenamefont {Pieronek}, \citenamefont {de~Raadt},
  \citenamefont {Steinke}, \citenamefont {Bin}, \citenamefont {Bulanov},
  \citenamefont {{van Tilborg}}, \citenamefont {Geddes}, \citenamefont
  {Schroeder}, \citenamefont {T{\'o}th}, \citenamefont {Esarey}, \citenamefont
  {Swanson}, \citenamefont {Fan-Chiang}, \citenamefont {Bagdasarov},
  \citenamefont {Bobrova}, \citenamefont {Gasilov}, \citenamefont {Korn},
  \citenamefont {Sasorov},\ and\ \citenamefont {Leemans}}]{Gonsalves.2019}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.~J.}\ \bibnamefont
  {Gonsalves}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Nakamura}},
  \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Daniels}}, \bibinfo
  {author} {\bibfnamefont {C.}~\bibnamefont {Benedetti}}, \bibinfo {author}
  {\bibfnamefont {C.}~\bibnamefont {Pieronek}}, \bibinfo {author}
  {\bibfnamefont {T.~C.~H.}\ \bibnamefont {de~Raadt}}, \bibinfo {author}
  {\bibfnamefont {S.}~\bibnamefont {Steinke}}, \bibinfo {author} {\bibfnamefont
  {J.~H.}\ \bibnamefont {Bin}}, \bibinfo {author} {\bibfnamefont {S.~S.}\
  \bibnamefont {Bulanov}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {{van Tilborg}}}, \bibinfo {author} {\bibfnamefont {C.~G.~R.}\ \bibnamefont
  {Geddes}}, \bibinfo {author} {\bibfnamefont {C.~B.}\ \bibnamefont
  {Schroeder}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {T{\'o}th}},
  \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Esarey}}, \bibinfo
  {author} {\bibfnamefont {K.}~\bibnamefont {Swanson}}, \bibinfo {author}
  {\bibfnamefont {L.}~\bibnamefont {Fan-Chiang}}, \bibinfo {author}
  {\bibfnamefont {G.}~\bibnamefont {Bagdasarov}}, \bibinfo {author}
  {\bibfnamefont {N.}~\bibnamefont {Bobrova}}, \bibinfo {author} {\bibfnamefont
  {V.}~\bibnamefont {Gasilov}}, \bibinfo {author} {\bibfnamefont
  {G.}~\bibnamefont {Korn}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont
  {Sasorov}},\ and\ \bibinfo {author} {\bibfnamefont {W.~P.}\ \bibnamefont
  {Leemans}},\ }\bibfield  {title} {\bibinfo {title} {{Petawatt Laser Guiding
  and Electron Beam Acceleration to 8 GeV in a Laser-Heated Capillary Discharge
  Waveguide}},\ }\href {https://doi.org/10.1103/PhysRevLett.122.084801}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {122}},\ \bibinfo {pages} {084801} (\bibinfo {year}
  {2019})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wang}\ \emph {et~al.}(2021)\citenamefont {Wang},
  \citenamefont {Feng}, \citenamefont {Ke}, \citenamefont {Yu}, \citenamefont
  {Xu}, \citenamefont {Qi}, \citenamefont {Chen}, \citenamefont {Qin},
  \citenamefont {Zhang}, \citenamefont {Fang}, \citenamefont {Liu},
  \citenamefont {Jiang}, \citenamefont {Wang}, \citenamefont {Wang},
  \citenamefont {Yang}, \citenamefont {Wu}, \citenamefont {Leng}, \citenamefont
  {Liu}, \citenamefont {Li},\ and\ \citenamefont {Xu}}]{Wang.2021}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {W.}~\bibnamefont
  {Wang}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Feng}}, \bibinfo
  {author} {\bibfnamefont {L.}~\bibnamefont {Ke}}, \bibinfo {author}
  {\bibfnamefont {C.}~\bibnamefont {Yu}}, \bibinfo {author} {\bibfnamefont
  {Y.}~\bibnamefont {Xu}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {Qi}}, \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Chen}}, \bibinfo
  {author} {\bibfnamefont {Z.}~\bibnamefont {Qin}}, \bibinfo {author}
  {\bibfnamefont {Z.}~\bibnamefont {Zhang}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Fang}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Liu}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Jiang}}, \bibinfo
  {author} {\bibfnamefont {H.}~\bibnamefont {Wang}}, \bibinfo {author}
  {\bibfnamefont {C.}~\bibnamefont {Wang}}, \bibinfo {author} {\bibfnamefont
  {X.}~\bibnamefont {Yang}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Wu}}, \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Leng}}, \bibinfo
  {author} {\bibfnamefont {J.}~\bibnamefont {Liu}}, \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {Li}},\ and\ \bibinfo {author}
  {\bibfnamefont {Z.}~\bibnamefont {Xu}},\ }\bibfield  {title} {\bibinfo
  {title} {{Free-electron lasing at 27 nanometres based on a laser wakefield
  accelerator}},\ }\href {https://doi.org/10.1038/s41586-021-03678-x}
  {\bibfield  {journal} {\bibinfo  {journal} {Nature}\ }\textbf {\bibinfo
  {volume} {595}},\ \bibinfo {pages} {516} (\bibinfo {year}
  {2021})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Fuchs}\ \emph {et~al.}(2009)\citenamefont {Fuchs},
  \citenamefont {Weingartner}, \citenamefont {Popp}, \citenamefont {Major},
  \citenamefont {Becker}, \citenamefont {Osterhoff}, \citenamefont {Cortrie},
  \citenamefont {Zeitler}, \citenamefont {H{\"o}rlein}, \citenamefont
  {Tsakiris}, \citenamefont {Schramm}, \citenamefont {Rowlands-Rees},
  \citenamefont {Hooker}, \citenamefont {Habs}, \citenamefont {Krausz},
  \citenamefont {Karsch},\ and\ \citenamefont {Gr{\"u}ner}}]{Fuchs.2009}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Fuchs}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Weingartner}},
  \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Popp}}, \bibinfo {author}
  {\bibfnamefont {Z.}~\bibnamefont {Major}}, \bibinfo {author} {\bibfnamefont
  {S.}~\bibnamefont {Becker}}, \bibinfo {author} {\bibfnamefont
  {J.}~\bibnamefont {Osterhoff}}, \bibinfo {author} {\bibfnamefont
  {I.}~\bibnamefont {Cortrie}}, \bibinfo {author} {\bibfnamefont
  {B.}~\bibnamefont {Zeitler}}, \bibinfo {author} {\bibfnamefont
  {R.}~\bibnamefont {H{\"o}rlein}}, \bibinfo {author} {\bibfnamefont {G.~D.}\
  \bibnamefont {Tsakiris}}, \bibinfo {author} {\bibfnamefont {U.}~\bibnamefont
  {Schramm}}, \bibinfo {author} {\bibfnamefont {T.~P.}\ \bibnamefont
  {Rowlands-Rees}}, \bibinfo {author} {\bibfnamefont {S.~M.}\ \bibnamefont
  {Hooker}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Habs}},
  \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Krausz}}, \bibinfo
  {author} {\bibfnamefont {S.}~\bibnamefont {Karsch}},\ and\ \bibinfo {author}
  {\bibfnamefont {F.}~\bibnamefont {Gr{\"u}ner}},\ }\bibfield  {title}
  {\bibinfo {title} {{Laser-driven soft-X-ray undulator source}},\ }\href
  {https://doi.org/10.1038/nphys1404} {\bibfield  {journal} {\bibinfo
  {journal} {Nat. Phys.}\ }\textbf {\bibinfo {volume} {5}},\ \bibinfo {pages}
  {826} (\bibinfo {year} {2009})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Huang}\ \emph {et~al.}(2012)\citenamefont {Huang},
  \citenamefont {Ding},\ and\ \citenamefont {Schroeder}}]{Huang.2012}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Z.}~\bibnamefont
  {Huang}}, \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Ding}},\ and\
  \bibinfo {author} {\bibfnamefont {C.~B.}\ \bibnamefont {Schroeder}},\
  }\bibfield  {title} {\bibinfo {title} {{Compact x-ray free-electron laser
  from a laser-plasma accelerator using a transverse-gradient undulator}},\
  }\href {https://doi.org/10.1103/PhysRevLett.109.204801} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {109}},\
  \bibinfo {pages} {204801} (\bibinfo {year} {2012})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Maier}\ \emph {et~al.}(2012)\citenamefont {Maier},
  \citenamefont {Meseck}, \citenamefont {Reiche}, \citenamefont {Schroeder},
  \citenamefont {Seggebrock},\ and\ \citenamefont {Gr{\"u}ner}}]{Maier.2012}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.~R.}\ \bibnamefont
  {Maier}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Meseck}},
  \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Reiche}}, \bibinfo
  {author} {\bibfnamefont {C.~B.}\ \bibnamefont {Schroeder}}, \bibinfo {author}
  {\bibfnamefont {T.}~\bibnamefont {Seggebrock}},\ and\ \bibinfo {author}
  {\bibfnamefont {F.}~\bibnamefont {Gr{\"u}ner}},\ }\bibfield  {title}
  {\bibinfo {title} {{Demonstration Scheme for a Laser-Plasma-Driven
  Free-Electron Laser}},\ }\href {https://doi.org/10.1103/PhysRevX.2.031019}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. X}\ }\textbf {\bibinfo
  {volume} {2}},\ \bibinfo {pages} {031019} (\bibinfo {year}
  {2012})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Leemans}\ and\ \citenamefont
  {Esarey}(2009)}]{Leemans.2009}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {W.}~\bibnamefont
  {Leemans}}\ and\ \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Esarey}},\ }\bibfield  {title} {\bibinfo {title} {{Laser-driven plasma-wave
  electron accelerators}},\ }\href {https://doi.org/10.1063/1.3099645}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Today}\ }\textbf {\bibinfo
  {volume} {62}},\ \bibinfo {pages} {44} (\bibinfo {year} {2009})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Schroeder}\ \emph {et~al.}(2010)\citenamefont
  {Schroeder}, \citenamefont {Esarey}, \citenamefont {Geddes}, \citenamefont
  {Benedetti},\ and\ \citenamefont {Leemans}}]{Schroeder.2010}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.~B.}\ \bibnamefont
  {Schroeder}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Esarey}},
  \bibinfo {author} {\bibfnamefont {C.~G.~R.}\ \bibnamefont {Geddes}}, \bibinfo
  {author} {\bibfnamefont {C.}~\bibnamefont {Benedetti}},\ and\ \bibinfo
  {author} {\bibfnamefont {W.~P.}\ \bibnamefont {Leemans}},\ }\bibfield
  {title} {\bibinfo {title} {{Physics considerations for laser-plasma linear
  colliders}},\ }\href {https://doi.org/10.1103/PhysRevSTAB.13.101301}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Spec. Top. Accel
  Beams}\ }\textbf {\bibinfo {volume} {13}},\ \bibinfo {pages} {101301}
  (\bibinfo {year} {2010})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {{ALEGRO
  collaboration}}(2019)}]{alegrocollaboration2019advanced}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {{ALEGRO
  collaboration}}},\ }\href {https://doi.org/10.48550/arXiv.1901.10370}
  {\bibinfo {title} {Towards an advanced linear international collider}}
  (\bibinfo {year} {2019}),\ \Eprint {https://arxiv.org/abs/1901.10370}
  {arXiv:1901.10370 [physics.acc-ph]} \BibitemShut {NoStop}%
\bibitem [{\citenamefont {Assmann}\ \emph {et~al.}(2020)\citenamefont
  {Assmann}, \citenamefont {Weikum}, \citenamefont {Akhter}, \citenamefont
  {Alesini}, \citenamefont {Alexandrova}, \citenamefont {Anania}, \citenamefont
  {Andreev}, \citenamefont {Andriyash}, \citenamefont {Artioli}, \citenamefont
  {Aschikhin}, \citenamefont {Audet}, \citenamefont {Bacci}, \citenamefont
  {Barna}, \citenamefont {Bartocci}, \citenamefont {Bayramian}, \citenamefont
  {Beaton}, \citenamefont {Beck}, \citenamefont {Bellaveglia}, \citenamefont
  {Beluze}, \citenamefont {Bernhard}, \citenamefont {Biagioni}, \citenamefont
  {Bielawski}, \citenamefont {Bisesto}, \citenamefont {Bonatto}, \citenamefont
  {Boulton}, \citenamefont {Brandi}, \citenamefont {Brinkmann}, \citenamefont
  {Briquez}, \citenamefont {Brottier}, \citenamefont {Br{\"u}ndermann},
  \citenamefont {B{\"u}scher}, \citenamefont {Buonomo}, \citenamefont
  {Bussmann}, \citenamefont {Bussolino}, \citenamefont {Campana}, \citenamefont
  {Cantarella}, \citenamefont {Cassou}, \citenamefont {Chanc{\'e}},
  \citenamefont {Chen}, \citenamefont {Chiadroni}, \citenamefont {Cianchi},
  \citenamefont {Cioeta}, \citenamefont {Clarke}, \citenamefont {Cole},
  \citenamefont {Costa}, \citenamefont {Couprie}, \citenamefont {Cowley},
  \citenamefont {Croia}, \citenamefont {Cros}, \citenamefont {Crump},
  \citenamefont {D'Arcy}, \citenamefont {Dattoli}, \citenamefont {{Del Dotto}},
  \citenamefont {Delerue}, \citenamefont {{Del Franco}}, \citenamefont
  {Delinikolas}, \citenamefont {de~Nicola}, \citenamefont {Dias}, \citenamefont
  {{Di Giovenale}}, \citenamefont {Diomede}, \citenamefont {{Di Pasquale}},
  \citenamefont {{Di Pirro}}, \citenamefont {{Di Raddo}}, \citenamefont
  {Dorda}, \citenamefont {Erlandson}, \citenamefont {Ertel}, \citenamefont
  {Esposito}, \citenamefont {Falcoz}, \citenamefont {Falone}, \citenamefont
  {Fedele}, \citenamefont {{Ferran Pousa}}, \citenamefont {Ferrario},
  \citenamefont {Filippi}, \citenamefont {Fils}, \citenamefont {Fiore},
  \citenamefont {Fiorito}, \citenamefont {Fonseca}, \citenamefont {Franzini},
  \citenamefont {Galimberti}, \citenamefont {Gallo}, \citenamefont {Galvin},
  \citenamefont {Ghaith}, \citenamefont {Ghigo}, \citenamefont {Giove},
  \citenamefont {Giribono}, \citenamefont {Gizzi}, \citenamefont {Gr{\"u}ner},
  \citenamefont {Habib}, \citenamefont {Haefner}, \citenamefont {Heinemann},
  \citenamefont {Helm}, \citenamefont {Hidding}, \citenamefont {Holzer},
  \citenamefont {Hooker}, \citenamefont {Hosokai}, \citenamefont {H{\"u}bner},
  \citenamefont {Ibison}, \citenamefont {Incremona}, \citenamefont {Irman},
  \citenamefont {Iungo}, \citenamefont {Jafarinia}, \citenamefont {Jakobsson},
  \citenamefont {Jaroszynski}, \citenamefont {Jaster-Merz}, \citenamefont
  {Joshi}, \citenamefont {Kaluza}, \citenamefont {Kando}, \citenamefont
  {Karger}, \citenamefont {Karsch}, \citenamefont {Khazanov}, \citenamefont
  {Khikhlukha}, \citenamefont {Kirchen}, \citenamefont {Kirwan}, \citenamefont
  {Kit{\'e}gi}, \citenamefont {Knetsch}, \citenamefont {Kocon}, \citenamefont
  {Koester}, \citenamefont {Kononenko}, \citenamefont {Korn}, \citenamefont
  {Kostyukov}, \citenamefont {Kruchinin}, \citenamefont {Labate}, \citenamefont
  {{Le Blanc}}, \citenamefont {Lechner}, \citenamefont {Lee}, \citenamefont
  {Leemans}, \citenamefont {Lehrach}, \citenamefont {Li}, \citenamefont {Li},
  \citenamefont {Libov}, \citenamefont {Lifschitz}, \citenamefont
  {Lindstr{\o}m}, \citenamefont {Litvinenko}, \citenamefont {Lu}, \citenamefont
  {Lundh}, \citenamefont {Maier}, \citenamefont {Malka}, \citenamefont
  {Manahan}, \citenamefont {Mangles}, \citenamefont {Marcelli}, \citenamefont
  {Marchetti}, \citenamefont {Marcouill{\'e}}, \citenamefont {Marocchino},
  \citenamefont {Marteau}, \citenamefont {{La Martinez de Ossa}}, \citenamefont
  {Martins}, \citenamefont {Mason}, \citenamefont {Massimo}, \citenamefont
  {Mathieu}, \citenamefont {Maynard}, \citenamefont {Mazzotta}, \citenamefont
  {Mironov}, \citenamefont {Molodozhentsev}, \citenamefont {Morante},
  \citenamefont {Mosnier}, \citenamefont {Mostacci}, \citenamefont
  {M{\"u}ller}, \citenamefont {Murphy}, \citenamefont {Najmudin}, \citenamefont
  {Nghiem}, \citenamefont {Nguyen}, \citenamefont {Niknejadi}, \citenamefont
  {Nutter}, \citenamefont {Osterhoff}, \citenamefont {{Oumbarek Espinos}},
  \citenamefont {Paillard}, \citenamefont {Papadopoulos}, \citenamefont
  {Patrizi}, \citenamefont {Pattathil}, \citenamefont {Pellegrino},
  \citenamefont {Petralia}, \citenamefont {Petrillo}, \citenamefont
  {Piersanti}, \citenamefont {Pocsai}, \citenamefont {Poder}, \citenamefont
  {Pompili}, \citenamefont {Pribyl}, \citenamefont {Pugacheva}, \citenamefont
  {Reagan}, \citenamefont {Resta-Lopez}, \citenamefont {Ricci}, \citenamefont
  {Romeo}, \citenamefont {{Rossetti Conti}}, \citenamefont {Rossi},
  \citenamefont {Rossmanith}, \citenamefont {Rotundo}, \citenamefont {Roussel},
  \citenamefont {Sabbatini}, \citenamefont {Santangelo}, \citenamefont {Sarri},
  \citenamefont {Schaper}, \citenamefont {Scherkl}, \citenamefont {Schramm},
  \citenamefont {Schroeder}, \citenamefont {Scifo}, \citenamefont {Serafini},
  \citenamefont {Sharma}, \citenamefont {Sheng}, \citenamefont {Shpakov},
  \citenamefont {Siders}, \citenamefont {Silva}, \citenamefont {Silva},
  \citenamefont {Simon}, \citenamefont {Simon-Boisson}, \citenamefont {Sinha},
  \citenamefont {Sistrunk}, \citenamefont {Specka}, \citenamefont {Spinka},
  \citenamefont {Stecchi}, \citenamefont {Stella}, \citenamefont {Stellato},
  \citenamefont {Streeter}, \citenamefont {Sutherland}, \citenamefont
  {Svystun}, \citenamefont {Symes}, \citenamefont {Szwaj}, \citenamefont
  {Tauscher}, \citenamefont {Terzani}, \citenamefont {Toci}, \citenamefont
  {Tomassini}, \citenamefont {Torres}, \citenamefont {Ullmann}, \citenamefont
  {Vaccarezza}, \citenamefont {Vall{\'e}au}, \citenamefont {Vannini},
  \citenamefont {Vannozzi}, \citenamefont {Vescovi}, \citenamefont {Vieira},
  \citenamefont {Villa}, \citenamefont {Wahlstr{\"o}m}, \citenamefont
  {Walczak}, \citenamefont {Walker}, \citenamefont {Wang}, \citenamefont
  {Welsch}, \citenamefont {Welsch}, \citenamefont {Weng}, \citenamefont
  {Wiggins}, \citenamefont {Wolfenden}, \citenamefont {Xia}, \citenamefont
  {Yabashi}, \citenamefont {Zhang}, \citenamefont {Zhao}, \citenamefont {Zhu},\
  and\ \citenamefont {Zigler}}]{Assmann.2020}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R.~W.}\ \bibnamefont
  {Assmann}}, \bibinfo {author} {\bibfnamefont {M.~K.}\ \bibnamefont {Weikum}},
  \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Akhter}}, \bibinfo
  {author} {\bibfnamefont {D.}~\bibnamefont {Alesini}}, \bibinfo {author}
  {\bibfnamefont {A.~S.}\ \bibnamefont {Alexandrova}}, \bibinfo {author}
  {\bibfnamefont {M.~P.}\ \bibnamefont {Anania}}, \bibinfo {author}
  {\bibfnamefont {N.~E.}\ \bibnamefont {Andreev}}, \bibinfo {author}
  {\bibfnamefont {I.}~\bibnamefont {Andriyash}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Artioli}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Aschikhin}}, \bibinfo {author} {\bibfnamefont
  {T.}~\bibnamefont {Audet}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Bacci}}, \bibinfo {author} {\bibfnamefont {I.~F.}\
  \bibnamefont {Barna}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Bartocci}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Bayramian}},
  \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Beaton}}, \bibinfo
  {author} {\bibfnamefont {A.}~\bibnamefont {Beck}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Bellaveglia}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Beluze}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Bernhard}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Biagioni}}, \bibinfo {author} {\bibfnamefont
  {S.}~\bibnamefont {Bielawski}}, \bibinfo {author} {\bibfnamefont {F.~G.}\
  \bibnamefont {Bisesto}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Bonatto}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Boulton}},
  \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Brandi}}, \bibinfo
  {author} {\bibfnamefont {R.}~\bibnamefont {Brinkmann}}, \bibinfo {author}
  {\bibfnamefont {F.}~\bibnamefont {Briquez}}, \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Brottier}}, \bibinfo {author} {\bibfnamefont
  {E.}~\bibnamefont {Br{\"u}ndermann}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {B{\"u}scher}}, \bibinfo {author} {\bibfnamefont
  {B.}~\bibnamefont {Buonomo}}, \bibinfo {author} {\bibfnamefont {M.~H.}\
  \bibnamefont {Bussmann}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Bussolino}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Campana}},
  \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Cantarella}}, \bibinfo
  {author} {\bibfnamefont {K.}~\bibnamefont {Cassou}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Chanc{\'e}}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Chen}}, \bibinfo {author} {\bibfnamefont
  {E.}~\bibnamefont {Chiadroni}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Cianchi}}, \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Cioeta}}, \bibinfo {author} {\bibfnamefont {J.~A.}\
  \bibnamefont {Clarke}}, \bibinfo {author} {\bibfnamefont {J.~M.}\
  \bibnamefont {Cole}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Costa}}, \bibinfo {author} {\bibfnamefont {M.-E.}\ \bibnamefont {Couprie}},
  \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Cowley}}, \bibinfo
  {author} {\bibfnamefont {M.}~\bibnamefont {Croia}}, \bibinfo {author}
  {\bibfnamefont {B.}~\bibnamefont {Cros}}, \bibinfo {author} {\bibfnamefont
  {P.~A.}\ \bibnamefont {Crump}}, \bibinfo {author} {\bibfnamefont
  {R.}~\bibnamefont {D'Arcy}}, \bibinfo {author} {\bibfnamefont
  {G.}~\bibnamefont {Dattoli}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {{Del Dotto}}}, \bibinfo {author} {\bibfnamefont
  {N.}~\bibnamefont {Delerue}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {{Del Franco}}}, \bibinfo {author} {\bibfnamefont
  {P.}~\bibnamefont {Delinikolas}}, \bibinfo {author} {\bibfnamefont
  {S.}~\bibnamefont {de~Nicola}}, \bibinfo {author} {\bibfnamefont {J.~M.}\
  \bibnamefont {Dias}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {{Di
  Giovenale}}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Diomede}},
  \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {{Di Pasquale}}}, \bibinfo
  {author} {\bibfnamefont {G.}~\bibnamefont {{Di Pirro}}}, \bibinfo {author}
  {\bibfnamefont {G.}~\bibnamefont {{Di Raddo}}}, \bibinfo {author}
  {\bibfnamefont {U.}~\bibnamefont {Dorda}}, \bibinfo {author} {\bibfnamefont
  {A.~C.}\ \bibnamefont {Erlandson}}, \bibinfo {author} {\bibfnamefont
  {K.}~\bibnamefont {Ertel}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Esposito}}, \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Falcoz}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Falone}}, \bibinfo {author} {\bibfnamefont
  {R.}~\bibnamefont {Fedele}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {{Ferran Pousa}}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Ferrario}}, \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Filippi}}, \bibinfo {author} {\bibfnamefont
  {J.}~\bibnamefont {Fils}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Fiore}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Fiorito}},
  \bibinfo {author} {\bibfnamefont {R.~A.}\ \bibnamefont {Fonseca}}, \bibinfo
  {author} {\bibfnamefont {G.}~\bibnamefont {Franzini}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Galimberti}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Gallo}}, \bibinfo {author} {\bibfnamefont
  {T.~C.}\ \bibnamefont {Galvin}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Ghaith}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Ghigo}}, \bibinfo {author} {\bibfnamefont
  {D.}~\bibnamefont {Giove}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Giribono}}, \bibinfo {author} {\bibfnamefont {L.~A.}\
  \bibnamefont {Gizzi}}, \bibinfo {author} {\bibfnamefont {F.~J.}\ \bibnamefont
  {Gr{\"u}ner}}, \bibinfo {author} {\bibfnamefont {A.~F.}\ \bibnamefont
  {Habib}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Haefner}},
  \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Heinemann}}, \bibinfo
  {author} {\bibfnamefont {A.}~\bibnamefont {Helm}}, \bibinfo {author}
  {\bibfnamefont {B.}~\bibnamefont {Hidding}}, \bibinfo {author} {\bibfnamefont
  {B.~J.}\ \bibnamefont {Holzer}}, \bibinfo {author} {\bibfnamefont {S.~M.}\
  \bibnamefont {Hooker}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont
  {Hosokai}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {H{\"u}bner}},
  \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Ibison}}, \bibinfo
  {author} {\bibfnamefont {S.}~\bibnamefont {Incremona}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Irman}}, \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Iungo}}, \bibinfo {author} {\bibfnamefont {F.~J.}\
  \bibnamefont {Jafarinia}}, \bibinfo {author} {\bibfnamefont {O.}~\bibnamefont
  {Jakobsson}}, \bibinfo {author} {\bibfnamefont {D.~A.}\ \bibnamefont
  {Jaroszynski}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Jaster-Merz}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Joshi}},
  \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Kaluza}}, \bibinfo
  {author} {\bibfnamefont {M.}~\bibnamefont {Kando}}, \bibinfo {author}
  {\bibfnamefont {O.~S.}\ \bibnamefont {Karger}}, \bibinfo {author}
  {\bibfnamefont {S.}~\bibnamefont {Karsch}}, \bibinfo {author} {\bibfnamefont
  {E.}~\bibnamefont {Khazanov}}, \bibinfo {author} {\bibfnamefont
  {D.}~\bibnamefont {Khikhlukha}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Kirchen}}, \bibinfo {author} {\bibfnamefont
  {G.}~\bibnamefont {Kirwan}}, \bibinfo {author} {\bibfnamefont
  {C.}~\bibnamefont {Kit{\'e}gi}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Knetsch}}, \bibinfo {author} {\bibfnamefont
  {D.}~\bibnamefont {Kocon}}, \bibinfo {author} {\bibfnamefont
  {P.}~\bibnamefont {Koester}}, \bibinfo {author} {\bibfnamefont {O.~S.}\
  \bibnamefont {Kononenko}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Korn}}, \bibinfo {author} {\bibfnamefont {I.}~\bibnamefont {Kostyukov}},
  \bibinfo {author} {\bibfnamefont {K.~O.}\ \bibnamefont {Kruchinin}}, \bibinfo
  {author} {\bibfnamefont {L.}~\bibnamefont {Labate}}, \bibinfo {author}
  {\bibfnamefont {C.}~\bibnamefont {{Le Blanc}}}, \bibinfo {author}
  {\bibfnamefont {C.}~\bibnamefont {Lechner}}, \bibinfo {author} {\bibfnamefont
  {P.}~\bibnamefont {Lee}}, \bibinfo {author} {\bibfnamefont {W.}~\bibnamefont
  {Leemans}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Lehrach}},
  \bibinfo {author} {\bibfnamefont {X.}~\bibnamefont {Li}}, \bibinfo {author}
  {\bibfnamefont {Y.}~\bibnamefont {Li}}, \bibinfo {author} {\bibfnamefont
  {V.}~\bibnamefont {Libov}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Lifschitz}}, \bibinfo {author} {\bibfnamefont {C.~A.}\
  \bibnamefont {Lindstr{\o}m}}, \bibinfo {author} {\bibfnamefont
  {V.}~\bibnamefont {Litvinenko}}, \bibinfo {author} {\bibfnamefont
  {W.}~\bibnamefont {Lu}}, \bibinfo {author} {\bibfnamefont {O.}~\bibnamefont
  {Lundh}}, \bibinfo {author} {\bibfnamefont {A.~R.}\ \bibnamefont {Maier}},
  \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Malka}}, \bibinfo
  {author} {\bibfnamefont {G.~G.}\ \bibnamefont {Manahan}}, \bibinfo {author}
  {\bibfnamefont {S.~P.~D.}\ \bibnamefont {Mangles}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Marcelli}}, \bibinfo {author}
  {\bibfnamefont {B.}~\bibnamefont {Marchetti}}, \bibinfo {author}
  {\bibfnamefont {O.}~\bibnamefont {Marcouill{\'e}}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Marocchino}}, \bibinfo {author}
  {\bibfnamefont {F.}~\bibnamefont {Marteau}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {{La Martinez de Ossa}}}, \bibinfo {author} {\bibfnamefont
  {J.~L.}\ \bibnamefont {Martins}}, \bibinfo {author} {\bibfnamefont {P.~D.}\
  \bibnamefont {Mason}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Massimo}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Mathieu}},
  \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Maynard}}, \bibinfo
  {author} {\bibfnamefont {Z.}~\bibnamefont {Mazzotta}}, \bibinfo {author}
  {\bibfnamefont {S.}~\bibnamefont {Mironov}}, \bibinfo {author} {\bibfnamefont
  {A.~Y.}\ \bibnamefont {Molodozhentsev}}, \bibinfo {author} {\bibfnamefont
  {S.}~\bibnamefont {Morante}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Mosnier}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Mostacci}}, \bibinfo {author} {\bibfnamefont {A.-S.}\
  \bibnamefont {M{\"u}ller}}, \bibinfo {author} {\bibfnamefont {C.~D.}\
  \bibnamefont {Murphy}}, \bibinfo {author} {\bibfnamefont {Z.}~\bibnamefont
  {Najmudin}}, \bibinfo {author} {\bibfnamefont {P.~A.~P.}\ \bibnamefont
  {Nghiem}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Nguyen}},
  \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Niknejadi}}, \bibinfo
  {author} {\bibfnamefont {A.}~\bibnamefont {Nutter}}, \bibinfo {author}
  {\bibfnamefont {J.}~\bibnamefont {Osterhoff}}, \bibinfo {author}
  {\bibfnamefont {D.}~\bibnamefont {{Oumbarek Espinos}}}, \bibinfo {author}
  {\bibfnamefont {J.-L.}\ \bibnamefont {Paillard}}, \bibinfo {author}
  {\bibfnamefont {D.~N.}\ \bibnamefont {Papadopoulos}}, \bibinfo {author}
  {\bibfnamefont {B.}~\bibnamefont {Patrizi}}, \bibinfo {author} {\bibfnamefont
  {R.}~\bibnamefont {Pattathil}}, \bibinfo {author} {\bibfnamefont
  {L.}~\bibnamefont {Pellegrino}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Petralia}}, \bibinfo {author} {\bibfnamefont
  {V.}~\bibnamefont {Petrillo}}, \bibinfo {author} {\bibfnamefont
  {L.}~\bibnamefont {Piersanti}}, \bibinfo {author} {\bibfnamefont {M.~A.}\
  \bibnamefont {Pocsai}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont
  {Poder}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Pompili}},
  \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Pribyl}}, \bibinfo
  {author} {\bibfnamefont {D.}~\bibnamefont {Pugacheva}}, \bibinfo {author}
  {\bibfnamefont {B.~A.}\ \bibnamefont {Reagan}}, \bibinfo {author}
  {\bibfnamefont {J.}~\bibnamefont {Resta-Lopez}}, \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {Ricci}}, \bibinfo {author} {\bibfnamefont
  {S.}~\bibnamefont {Romeo}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {{Rossetti Conti}}}, \bibinfo {author} {\bibfnamefont
  {A.~R.}\ \bibnamefont {Rossi}}, \bibinfo {author} {\bibfnamefont
  {R.}~\bibnamefont {Rossmanith}}, \bibinfo {author} {\bibfnamefont
  {U.}~\bibnamefont {Rotundo}}, \bibinfo {author} {\bibfnamefont
  {E.}~\bibnamefont {Roussel}}, \bibinfo {author} {\bibfnamefont
  {L.}~\bibnamefont {Sabbatini}}, \bibinfo {author} {\bibfnamefont
  {P.}~\bibnamefont {Santangelo}}, \bibinfo {author} {\bibfnamefont
  {G.}~\bibnamefont {Sarri}}, \bibinfo {author} {\bibfnamefont
  {L.}~\bibnamefont {Schaper}}, \bibinfo {author} {\bibfnamefont
  {P.}~\bibnamefont {Scherkl}}, \bibinfo {author} {\bibfnamefont
  {U.}~\bibnamefont {Schramm}}, \bibinfo {author} {\bibfnamefont {C.~B.}\
  \bibnamefont {Schroeder}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Scifo}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Serafini}},
  \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Sharma}}, \bibinfo
  {author} {\bibfnamefont {Z.~M.}\ \bibnamefont {Sheng}}, \bibinfo {author}
  {\bibfnamefont {V.}~\bibnamefont {Shpakov}}, \bibinfo {author} {\bibfnamefont
  {C.~W.}\ \bibnamefont {Siders}}, \bibinfo {author} {\bibfnamefont {L.~O.}\
  \bibnamefont {Silva}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont
  {Silva}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Simon}},
  \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Simon-Boisson}}, \bibinfo
  {author} {\bibfnamefont {U.}~\bibnamefont {Sinha}}, \bibinfo {author}
  {\bibfnamefont {E.}~\bibnamefont {Sistrunk}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Specka}}, \bibinfo {author} {\bibfnamefont
  {T.~M.}\ \bibnamefont {Spinka}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Stecchi}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Stella}}, \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Stellato}}, \bibinfo {author} {\bibfnamefont {M.~J.~V.}\
  \bibnamefont {Streeter}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Sutherland}}, \bibinfo {author} {\bibfnamefont {E.~N.}\ \bibnamefont
  {Svystun}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Symes}},
  \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Szwaj}}, \bibinfo
  {author} {\bibfnamefont {G.~E.}\ \bibnamefont {Tauscher}}, \bibinfo {author}
  {\bibfnamefont {D.}~\bibnamefont {Terzani}}, \bibinfo {author} {\bibfnamefont
  {G.}~\bibnamefont {Toci}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont
  {Tomassini}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Torres}},
  \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Ullmann}}, \bibinfo
  {author} {\bibfnamefont {C.}~\bibnamefont {Vaccarezza}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Vall{\'e}au}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Vannini}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Vannozzi}}, \bibinfo {author} {\bibfnamefont
  {S.}~\bibnamefont {Vescovi}}, \bibinfo {author} {\bibfnamefont {J.~M.}\
  \bibnamefont {Vieira}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Villa}}, \bibinfo {author} {\bibfnamefont {C.-G.}\ \bibnamefont
  {Wahlstr{\"o}m}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {Walczak}}, \bibinfo {author} {\bibfnamefont {P.~A.}\ \bibnamefont {Walker}},
  \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Wang}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Welsch}}, \bibinfo {author} {\bibfnamefont
  {C.~P.}\ \bibnamefont {Welsch}}, \bibinfo {author} {\bibfnamefont {S.~M.}\
  \bibnamefont {Weng}}, \bibinfo {author} {\bibfnamefont {S.~M.}\ \bibnamefont
  {Wiggins}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Wolfenden}},
  \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Xia}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Yabashi}}, \bibinfo {author} {\bibfnamefont
  {H.}~\bibnamefont {Zhang}}, \bibinfo {author} {\bibfnamefont
  {Y.}~\bibnamefont {Zhao}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Zhu}},\ and\ \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Zigler}},\
  }\bibfield  {title} {\bibinfo {title} {{EuPRAXIA Conceptual Design Report}},\
  }\href {https://doi.org/10.1140/epjst/e2020-000127-8} {\bibfield  {journal}
  {\bibinfo  {journal} {Eur. Phys. J. Spec. Top.}\ }\textbf {\bibinfo {volume}
  {229}},\ \bibinfo {pages} {3675} (\bibinfo {year} {2020})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Rousse}\ \emph {et~al.}(2004)\citenamefont {Rousse},
  \citenamefont {Phuoc}, \citenamefont {Shah}, \citenamefont {Pukhov},
  \citenamefont {Lefebvre}, \citenamefont {Malka}, \citenamefont {Kiselev},
  \citenamefont {Burgy}, \citenamefont {Rousseau}, \citenamefont {Umstadter},\
  and\ \citenamefont {Hulin}}]{Rousse.2004}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Rousse}}, \bibinfo {author} {\bibfnamefont {K.~T.}\ \bibnamefont {Phuoc}},
  \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Shah}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Pukhov}}, \bibinfo {author} {\bibfnamefont
  {E.}~\bibnamefont {Lefebvre}}, \bibinfo {author} {\bibfnamefont
  {V.}~\bibnamefont {Malka}}, \bibinfo {author} {\bibfnamefont
  {S.}~\bibnamefont {Kiselev}}, \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Burgy}}, \bibinfo {author} {\bibfnamefont {J.-P.}\
  \bibnamefont {Rousseau}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {Umstadter}},\ and\ \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {Hulin}},\ }\bibfield  {title} {\bibinfo {title} {{Production of a keV x-ray
  beam from synchrotron radiation in relativistic laser-plasma interaction}},\
  }\href {https://doi.org/10.1103/PhysRevLett.93.135005} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {93}},\
  \bibinfo {pages} {135005} (\bibinfo {year} {2004})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Jaroszynski}\ \emph {et~al.}(2006)\citenamefont
  {Jaroszynski}, \citenamefont {Bingham}, \citenamefont {Brunetti},
  \citenamefont {Ersfeld}, \citenamefont {Gallacher}, \citenamefont {{van der
  Geer}}, \citenamefont {Issac}, \citenamefont {Jamison}, \citenamefont
  {Jones}, \citenamefont {de~Loos}, \citenamefont {Lyachev}, \citenamefont
  {Pavlov}, \citenamefont {Reitsma}, \citenamefont {Saveliev}, \citenamefont
  {Vieux},\ and\ \citenamefont {Wiggins}}]{Jaroszynski.2006}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.~A.}\ \bibnamefont
  {Jaroszynski}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {Bingham}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Brunetti}},
  \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Ersfeld}}, \bibinfo
  {author} {\bibfnamefont {J.}~\bibnamefont {Gallacher}}, \bibinfo {author}
  {\bibfnamefont {B.}~\bibnamefont {{van der Geer}}}, \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {Issac}}, \bibinfo {author} {\bibfnamefont
  {S.~P.}\ \bibnamefont {Jamison}}, \bibinfo {author} {\bibfnamefont
  {D.}~\bibnamefont {Jones}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {de~Loos}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Lyachev}}, \bibinfo {author} {\bibfnamefont
  {V.}~\bibnamefont {Pavlov}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Reitsma}}, \bibinfo {author} {\bibfnamefont
  {Y.}~\bibnamefont {Saveliev}}, \bibinfo {author} {\bibfnamefont
  {G.}~\bibnamefont {Vieux}},\ and\ \bibinfo {author} {\bibfnamefont {S.~M.}\
  \bibnamefont {Wiggins}},\ }\bibfield  {title} {\bibinfo {title} {{Radiation
  sources based on laser-plasma interactions}},\ }\href
  {https://doi.org/10.1098/rsta.2005.1732} {\bibfield  {journal} {\bibinfo
  {journal} {Philos. Trans. R. Soc. London, Ser. A}\ }\textbf {\bibinfo
  {volume} {364}},\ \bibinfo {pages} {689} (\bibinfo {year}
  {2006})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kneip}\ \emph {et~al.}(2010)\citenamefont {Kneip},
  \citenamefont {McGuffey}, \citenamefont {Martins}, \citenamefont {Martins},
  \citenamefont {Bellei}, \citenamefont {Chvykov}, \citenamefont {Dollar},
  \citenamefont {Fonseca}, \citenamefont {Huntington}, \citenamefont
  {Kalintchenko}, \citenamefont {Maksimchuk}, \citenamefont {Mangles},
  \citenamefont {Matsuoka}, \citenamefont {Nagel}, \citenamefont {Palmer},
  \citenamefont {Schreiber}, \citenamefont {Phuoc}, \citenamefont {Thomas},
  \citenamefont {Yanovsky}, \citenamefont {Silva}, \citenamefont
  {Krushelnick},\ and\ \citenamefont {Najmudin}}]{Kneip.2010}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Kneip}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {McGuffey}},
  \bibinfo {author} {\bibfnamefont {J.~L.}\ \bibnamefont {Martins}}, \bibinfo
  {author} {\bibfnamefont {S.~F.}\ \bibnamefont {Martins}}, \bibinfo {author}
  {\bibfnamefont {C.}~\bibnamefont {Bellei}}, \bibinfo {author} {\bibfnamefont
  {V.}~\bibnamefont {Chvykov}}, \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Dollar}}, \bibinfo {author} {\bibfnamefont
  {R.}~\bibnamefont {Fonseca}}, \bibinfo {author} {\bibfnamefont
  {C.}~\bibnamefont {Huntington}}, \bibinfo {author} {\bibfnamefont
  {G.}~\bibnamefont {Kalintchenko}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Maksimchuk}}, \bibinfo {author} {\bibfnamefont {S.~P.~D.}\
  \bibnamefont {Mangles}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont
  {Matsuoka}}, \bibinfo {author} {\bibfnamefont {S.~R.}\ \bibnamefont {Nagel}},
  \bibinfo {author} {\bibfnamefont {C.~A.~J.}\ \bibnamefont {Palmer}}, \bibinfo
  {author} {\bibfnamefont {J.}~\bibnamefont {Schreiber}}, \bibinfo {author}
  {\bibfnamefont {K.~T.}\ \bibnamefont {Phuoc}}, \bibinfo {author}
  {\bibfnamefont {A.~G.~R.}\ \bibnamefont {Thomas}}, \bibinfo {author}
  {\bibfnamefont {V.}~\bibnamefont {Yanovsky}}, \bibinfo {author}
  {\bibfnamefont {L.~O.}\ \bibnamefont {Silva}}, \bibinfo {author}
  {\bibfnamefont {K.}~\bibnamefont {Krushelnick}},\ and\ \bibinfo {author}
  {\bibfnamefont {Z.}~\bibnamefont {Najmudin}},\ }\bibfield  {title} {\bibinfo
  {title} {{Bright spatially coherent synchrotron X-rays from a table-top
  source}},\ }\href {https://doi.org/10.1038/nphys1789} {\bibfield  {journal}
  {\bibinfo  {journal} {Nature Phys.}\ }\textbf {\bibinfo {volume} {6}},\
  \bibinfo {pages} {980} (\bibinfo {year} {2010})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Geddes}\ \emph {et~al.}(2015)\citenamefont {Geddes},
  \citenamefont {Rykovanov}, \citenamefont {Matlis}, \citenamefont {Steinke},
  \citenamefont {Vay}, \citenamefont {Esarey}, \citenamefont {Ludewigt},
  \citenamefont {Nakamura}, \citenamefont {Quiter}, \citenamefont {Schroeder},
  \citenamefont {Toth},\ and\ \citenamefont {Leemans}}]{Geddes.2015}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.~G.}\ \bibnamefont
  {Geddes}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Rykovanov}},
  \bibinfo {author} {\bibfnamefont {N.~H.}\ \bibnamefont {Matlis}}, \bibinfo
  {author} {\bibfnamefont {S.}~\bibnamefont {Steinke}}, \bibinfo {author}
  {\bibfnamefont {J.-L.}\ \bibnamefont {Vay}}, \bibinfo {author} {\bibfnamefont
  {E.~H.}\ \bibnamefont {Esarey}}, \bibinfo {author} {\bibfnamefont
  {B.}~\bibnamefont {Ludewigt}}, \bibinfo {author} {\bibfnamefont
  {K.}~\bibnamefont {Nakamura}}, \bibinfo {author} {\bibfnamefont {B.~J.}\
  \bibnamefont {Quiter}}, \bibinfo {author} {\bibfnamefont {C.~B.}\
  \bibnamefont {Schroeder}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont
  {Toth}},\ and\ \bibinfo {author} {\bibfnamefont {W.~P.}\ \bibnamefont
  {Leemans}},\ }\bibfield  {title} {\bibinfo {title} {{Compact
  quasi-monoenergetic photon sources from laser-plasma accelerators for nuclear
  detection and characterization}},\ }\href
  {https://doi.org/10.1016/j.nimb.2015.01.013} {\bibfield  {journal} {\bibinfo
  {journal} {Nucl. Instrum. Methods Phys. Res., Sect. B}\ }\textbf {\bibinfo
  {volume} {350}},\ \bibinfo {pages} {116} (\bibinfo {year}
  {2015})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Powers}\ \emph {et~al.}(2014)\citenamefont {Powers},
  \citenamefont {Ghebregziabher}, \citenamefont {Golovin}, \citenamefont {Liu},
  \citenamefont {Chen}, \citenamefont {Banerjee}, \citenamefont {Zhang},\ and\
  \citenamefont {Umstadter}}]{Powers.2014}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {N.~D.}\ \bibnamefont
  {Powers}}, \bibinfo {author} {\bibfnamefont {I.}~\bibnamefont
  {Ghebregziabher}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Golovin}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Liu}},
  \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Chen}}, \bibinfo {author}
  {\bibfnamefont {S.}~\bibnamefont {Banerjee}}, \bibinfo {author}
  {\bibfnamefont {J.}~\bibnamefont {Zhang}},\ and\ \bibinfo {author}
  {\bibfnamefont {D.~P.}\ \bibnamefont {Umstadter}},\ }\bibfield  {title}
  {\bibinfo {title} {{Quasi-monoenergetic and tunable X-rays from a
  laser-driven Compton light source}},\ }\href
  {https://doi.org/10.1038/nphoton.2013.314} {\bibfield  {journal} {\bibinfo
  {journal} {Nat. Photonics}\ }\textbf {\bibinfo {volume} {8}},\ \bibinfo
  {pages} {28} (\bibinfo {year} {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Cianchi}\ \emph {et~al.}(2016)\citenamefont
  {Cianchi}, \citenamefont {Anania}, \citenamefont {Bisesto}, \citenamefont
  {Castellano}, \citenamefont {Chiadroni}, \citenamefont {Pompili},\ and\
  \citenamefont {Shpakov}}]{Cianchi.2016}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Cianchi}}, \bibinfo {author} {\bibfnamefont {M.~P.}\ \bibnamefont {Anania}},
  \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Bisesto}}, \bibinfo
  {author} {\bibfnamefont {M.}~\bibnamefont {Castellano}}, \bibinfo {author}
  {\bibfnamefont {E.}~\bibnamefont {Chiadroni}}, \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {Pompili}},\ and\ \bibinfo {author}
  {\bibfnamefont {V.}~\bibnamefont {Shpakov}},\ }\bibfield  {title} {\bibinfo
  {title} {{Observations and diagnostics in high brightness beams}},\ }\href
  {https://doi.org/10.1016/j.nima.2016.03.076} {\bibfield  {journal} {\bibinfo
  {journal} {Nucl. Instrum. Methods Phys. Res., Sect. A}\ }\textbf {\bibinfo
  {volume} {829}},\ \bibinfo {pages} {343} (\bibinfo {year}
  {2016})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Pak}\ \emph {et~al.}(2010)\citenamefont {Pak},
  \citenamefont {Marsh}, \citenamefont {Martins}, \citenamefont {Lu},
  \citenamefont {Mori},\ and\ \citenamefont {Joshi}}]{Pak.2010}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Pak}}, \bibinfo {author} {\bibfnamefont {K.~A.}\ \bibnamefont {Marsh}},
  \bibinfo {author} {\bibfnamefont {S.~F.}\ \bibnamefont {Martins}}, \bibinfo
  {author} {\bibfnamefont {W.}~\bibnamefont {Lu}}, \bibinfo {author}
  {\bibfnamefont {W.~B.}\ \bibnamefont {Mori}},\ and\ \bibinfo {author}
  {\bibfnamefont {C.}~\bibnamefont {Joshi}},\ }\bibfield  {title} {\bibinfo
  {title} {{Injection and trapping of tunnel-ionized electrons into
  laser-produced wakes}},\ }\href
  {https://doi.org/10.1103/PhysRevLett.104.025003} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {104}},\
  \bibinfo {pages} {025003} (\bibinfo {year} {2010})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {McGuffey}\ \emph {et~al.}(2010)\citenamefont
  {McGuffey}, \citenamefont {Thomas}, \citenamefont {Schumaker}, \citenamefont
  {Matsuoka}, \citenamefont {Chvykov}, \citenamefont {Dollar}, \citenamefont
  {Kalintchenko}, \citenamefont {Yanovsky}, \citenamefont {Maksimchuk},
  \citenamefont {Krushelnick}, \citenamefont {Bychenkov}, \citenamefont
  {Glazyrin},\ and\ \citenamefont {Karpeev}}]{McGuffey.2010}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.}~\bibnamefont
  {McGuffey}}, \bibinfo {author} {\bibfnamefont {A.~G.~R.}\ \bibnamefont
  {Thomas}}, \bibinfo {author} {\bibfnamefont {W.}~\bibnamefont {Schumaker}},
  \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Matsuoka}}, \bibinfo
  {author} {\bibfnamefont {V.}~\bibnamefont {Chvykov}}, \bibinfo {author}
  {\bibfnamefont {F.~J.}\ \bibnamefont {Dollar}}, \bibinfo {author}
  {\bibfnamefont {G.}~\bibnamefont {Kalintchenko}}, \bibinfo {author}
  {\bibfnamefont {V.}~\bibnamefont {Yanovsky}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Maksimchuk}}, \bibinfo {author}
  {\bibfnamefont {K.}~\bibnamefont {Krushelnick}}, \bibinfo {author}
  {\bibfnamefont {V.~Y.}\ \bibnamefont {Bychenkov}}, \bibinfo {author}
  {\bibfnamefont {I.~V.}\ \bibnamefont {Glazyrin}},\ and\ \bibinfo {author}
  {\bibfnamefont {A.~V.}\ \bibnamefont {Karpeev}},\ }\bibfield  {title}
  {\bibinfo {title} {{Ionization induced trapping in a laser wakefield
  accelerator}},\ }\href {https://doi.org/10.1103/PhysRevLett.104.025004}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {104}},\ \bibinfo {pages} {025004} (\bibinfo {year}
  {2010})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Chien}\ \emph {et~al.}(2005)\citenamefont {Chien},
  \citenamefont {Chang}, \citenamefont {Lee}, \citenamefont {Lin},
  \citenamefont {Wang},\ and\ \citenamefont {Chen}}]{Chien.2005}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {T.-Y.}\ \bibnamefont
  {Chien}}, \bibinfo {author} {\bibfnamefont {C.-L.}\ \bibnamefont {Chang}},
  \bibinfo {author} {\bibfnamefont {C.-H.}\ \bibnamefont {Lee}}, \bibinfo
  {author} {\bibfnamefont {J.-Y.}\ \bibnamefont {Lin}}, \bibinfo {author}
  {\bibfnamefont {J.}~\bibnamefont {Wang}},\ and\ \bibinfo {author}
  {\bibfnamefont {S.-Y.}\ \bibnamefont {Chen}},\ }\bibfield  {title} {\bibinfo
  {title} {{Spatially localized self-injection of electrons in a self-modulated
  laser-wakefield accelerator by using a laser-induced transient density
  ramp}},\ }\href {https://doi.org/10.1103/PhysRevLett.94.115003} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {94}},\ \bibinfo {pages} {115003} (\bibinfo {year}
  {2005})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Weingartner}\ \emph {et~al.}(2012)\citenamefont
  {Weingartner}, \citenamefont {Raith}, \citenamefont {Popp}, \citenamefont
  {Chou}, \citenamefont {Wenz}, \citenamefont {Khrennikov}, \citenamefont
  {Heigoldt}, \citenamefont {Maier}, \citenamefont {Kajumba}, \citenamefont
  {Fuchs}, \citenamefont {Zeitler}, \citenamefont {Krausz}, \citenamefont
  {Karsch},\ and\ \citenamefont {Gr{\"u}ner}}]{Weingartner.2012}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {Weingartner}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Raith}},
  \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Popp}}, \bibinfo {author}
  {\bibfnamefont {S.}~\bibnamefont {Chou}}, \bibinfo {author} {\bibfnamefont
  {J.}~\bibnamefont {Wenz}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont
  {Khrennikov}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Heigoldt}}, \bibinfo {author} {\bibfnamefont {A.~R.}\ \bibnamefont {Maier}},
  \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont {Kajumba}}, \bibinfo
  {author} {\bibfnamefont {M.}~\bibnamefont {Fuchs}}, \bibinfo {author}
  {\bibfnamefont {B.}~\bibnamefont {Zeitler}}, \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Krausz}}, \bibinfo {author} {\bibfnamefont
  {S.}~\bibnamefont {Karsch}},\ and\ \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Gr{\"u}ner}},\ }\bibfield  {title} {\bibinfo {title}
  {{Ultralow emittance electron beams from a laser-wakefield accelerator}},\
  }\href {https://doi.org/10.1103/PhysRevSTAB.15.111302} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Spec. Top. Accel Beams}\ }\textbf {\bibinfo
  {volume} {15}},\ \bibinfo {pages} {111302} (\bibinfo {year}
  {2012})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Hidding}\ \emph {et~al.}(2012)\citenamefont
  {Hidding}, \citenamefont {Pretzler}, \citenamefont {Rosenzweig},
  \citenamefont {K{\"o}nigstein}, \citenamefont {Schiller},\ and\ \citenamefont
  {Bruhwiler}}]{Hidding.2012}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Hidding}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Pretzler}},
  \bibinfo {author} {\bibfnamefont {J.~B.}\ \bibnamefont {Rosenzweig}},
  \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {K{\"o}nigstein}},
  \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Schiller}},\ and\
  \bibinfo {author} {\bibfnamefont {D.~L.}\ \bibnamefont {Bruhwiler}},\
  }\bibfield  {title} {\bibinfo {title} {{Ultracold electron bunch generation
  via plasma photocathode emission and acceleration in a beam-driven plasma
  blowout}},\ }\href {https://doi.org/10.1103/PhysRevLett.108.035001}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {108}},\ \bibinfo {pages} {035001} (\bibinfo {year}
  {2012})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Li}\ \emph {et~al.}(2013)\citenamefont {Li},
  \citenamefont {Hua}, \citenamefont {Xu}, \citenamefont {Zhang}, \citenamefont
  {Yan}, \citenamefont {Du}, \citenamefont {Huang}, \citenamefont {Chen},
  \citenamefont {Tang}, \citenamefont {Lu}, \citenamefont {Joshi},
  \citenamefont {Mori},\ and\ \citenamefont {Gu}}]{Li.2013}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Li}}, \bibinfo {author} {\bibfnamefont {J.~F.}\ \bibnamefont {Hua}},
  \bibinfo {author} {\bibfnamefont {X.~L.}\ \bibnamefont {Xu}}, \bibinfo
  {author} {\bibfnamefont {C.~J.}\ \bibnamefont {Zhang}}, \bibinfo {author}
  {\bibfnamefont {L.~X.}\ \bibnamefont {Yan}}, \bibinfo {author} {\bibfnamefont
  {Y.~C.}\ \bibnamefont {Du}}, \bibinfo {author} {\bibfnamefont {W.~H.}\
  \bibnamefont {Huang}}, \bibinfo {author} {\bibfnamefont {H.~B.}\ \bibnamefont
  {Chen}}, \bibinfo {author} {\bibfnamefont {C.~X.}\ \bibnamefont {Tang}},
  \bibinfo {author} {\bibfnamefont {W.}~\bibnamefont {Lu}}, \bibinfo {author}
  {\bibfnamefont {C.}~\bibnamefont {Joshi}}, \bibinfo {author} {\bibfnamefont
  {W.~B.}\ \bibnamefont {Mori}},\ and\ \bibinfo {author} {\bibfnamefont
  {Y.~Q.}\ \bibnamefont {Gu}},\ }\bibfield  {title} {\bibinfo {title}
  {{Generating high-brightness electron beams via ionization injection by
  transverse colliding lasers in a plasma-wakefield accelerator}},\ }\href
  {https://doi.org/10.1103/PhysRevLett.111.015003} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {111}},\
  \bibinfo {pages} {015003} (\bibinfo {year} {2013})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wittig}\ \emph {et~al.}(2015)\citenamefont {Wittig},
  \citenamefont {Karger}, \citenamefont {Knetsch}, \citenamefont {Xi},
  \citenamefont {Deng}, \citenamefont {Rosenzweig}, \citenamefont {Bruhwiler},
  \citenamefont {Smith}, \citenamefont {Manahan}, \citenamefont {Sheng},
  \citenamefont {Jaroszynski},\ and\ \citenamefont {Hidding}}]{Wittig.2015}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Wittig}}, \bibinfo {author} {\bibfnamefont {O.}~\bibnamefont {Karger}},
  \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Knetsch}}, \bibinfo
  {author} {\bibfnamefont {Y.}~\bibnamefont {Xi}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Deng}}, \bibinfo {author} {\bibfnamefont
  {J.~B.}\ \bibnamefont {Rosenzweig}}, \bibinfo {author} {\bibfnamefont
  {D.~L.}\ \bibnamefont {Bruhwiler}}, \bibinfo {author} {\bibfnamefont
  {J.}~\bibnamefont {Smith}}, \bibinfo {author} {\bibfnamefont {G.~G.}\
  \bibnamefont {Manahan}}, \bibinfo {author} {\bibfnamefont {Z.-M.}\
  \bibnamefont {Sheng}}, \bibinfo {author} {\bibfnamefont {D.~A.}\ \bibnamefont
  {Jaroszynski}},\ and\ \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Hidding}},\ }\bibfield  {title} {\bibinfo {title} {{Optical plasma torch
  electron bunch generation in plasma wakefield accelerators}},\ }\href
  {https://doi.org/10.1103/PhysRevSTAB.18.081304} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. ST Accel. Beams}\ }\textbf {\bibinfo
  {volume} {18}},\ \bibinfo {pages} {081304} (\bibinfo {year}
  {2015})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Xu}\ \emph {et~al.}(2014)\citenamefont {Xu},
  \citenamefont {Hua}, \citenamefont {Li}, \citenamefont {Zhang}, \citenamefont
  {Yan}, \citenamefont {Du}, \citenamefont {Huang}, \citenamefont {Chen},
  \citenamefont {Tang}, \citenamefont {Lu}, \citenamefont {Yu}, \citenamefont
  {An}, \citenamefont {Joshi},\ and\ \citenamefont {Mori}}]{Xu.2014}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {X.~L.}\ \bibnamefont
  {Xu}}, \bibinfo {author} {\bibfnamefont {J.~F.}\ \bibnamefont {Hua}},
  \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Li}}, \bibinfo {author}
  {\bibfnamefont {C.~J.}\ \bibnamefont {Zhang}}, \bibinfo {author}
  {\bibfnamefont {L.~X.}\ \bibnamefont {Yan}}, \bibinfo {author} {\bibfnamefont
  {Y.~C.}\ \bibnamefont {Du}}, \bibinfo {author} {\bibfnamefont {W.~H.}\
  \bibnamefont {Huang}}, \bibinfo {author} {\bibfnamefont {H.~B.}\ \bibnamefont
  {Chen}}, \bibinfo {author} {\bibfnamefont {C.~X.}\ \bibnamefont {Tang}},
  \bibinfo {author} {\bibfnamefont {W.}~\bibnamefont {Lu}}, \bibinfo {author}
  {\bibfnamefont {P.}~\bibnamefont {Yu}}, \bibinfo {author} {\bibfnamefont
  {W.}~\bibnamefont {An}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont
  {Joshi}},\ and\ \bibinfo {author} {\bibfnamefont {W.~B.}\ \bibnamefont
  {Mori}},\ }\bibfield  {title} {\bibinfo {title} {{Phase-space dynamics of
  ionization injection in plasma-based accelerators}},\ }\href
  {https://doi.org/10.1103/PhysRevLett.112.035003} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {112}},\
  \bibinfo {pages} {035003} (\bibinfo {year} {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Manahan}\ \emph {et~al.}(2017)\citenamefont
  {Manahan}, \citenamefont {Habib}, \citenamefont {Scherkl}, \citenamefont
  {Delinikolas}, \citenamefont {Beaton}, \citenamefont {Knetsch}, \citenamefont
  {Karger}, \citenamefont {Wittig}, \citenamefont {Heinemann}, \citenamefont
  {Sheng}, \citenamefont {Cary}, \citenamefont {Bruhwiler}, \citenamefont
  {Rosenzweig},\ and\ \citenamefont {Hidding}}]{Manahan.2017}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.~G.}\ \bibnamefont
  {Manahan}}, \bibinfo {author} {\bibfnamefont {A.~F.}\ \bibnamefont {Habib}},
  \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Scherkl}}, \bibinfo
  {author} {\bibfnamefont {P.}~\bibnamefont {Delinikolas}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Beaton}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Knetsch}}, \bibinfo {author} {\bibfnamefont
  {O.}~\bibnamefont {Karger}}, \bibinfo {author} {\bibfnamefont
  {G.}~\bibnamefont {Wittig}}, \bibinfo {author} {\bibfnamefont
  {T.}~\bibnamefont {Heinemann}}, \bibinfo {author} {\bibfnamefont {Z.~M.}\
  \bibnamefont {Sheng}}, \bibinfo {author} {\bibfnamefont {J.~R.}\ \bibnamefont
  {Cary}}, \bibinfo {author} {\bibfnamefont {D.~L.}\ \bibnamefont {Bruhwiler}},
  \bibinfo {author} {\bibfnamefont {J.~B.}\ \bibnamefont {Rosenzweig}},\ and\
  \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Hidding}},\ }\bibfield
  {title} {\bibinfo {title} {{Single-stage plasma-based correlated energy
  spread compensation for ultrahigh 6D brightness electron beams}},\ }\href
  {https://doi.org/10.1038/ncomms15705} {\bibfield  {journal} {\bibinfo
  {journal} {Nat. Commun.}\ }\textbf {\bibinfo {volume} {8}},\ \bibinfo {pages}
  {15705} (\bibinfo {year} {2017})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Foster}\ \emph {et~al.}(2023)\citenamefont {Foster},
  \citenamefont {D'Arcy},\ and\ \citenamefont {Lindstr{\o}m}}]{Foster.2023}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Foster}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {D'Arcy}},\
  and\ \bibinfo {author} {\bibfnamefont {C.~A.}\ \bibnamefont {Lindstr{\o}m}},\
  }\bibfield  {title} {\bibinfo {title} {{A hybrid, asymmetric, linear Higgs
  factory based on plasma-wakefield and radio-frequency acceleration}},\ }\href
  {https://doi.org/10.1088/1367-2630/acf395} {\bibfield  {journal} {\bibinfo
  {journal} {New J. Phys.}\ }\textbf {\bibinfo {volume} {25}},\ \bibinfo
  {pages} {093037} (\bibinfo {year} {2023})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Akre}\ \emph {et~al.}(2001)\citenamefont {Akre},
  \citenamefont {Bentson}, \citenamefont {Emma},\ and\ \citenamefont
  {Krejcik}}]{Akre.2001}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {Akre}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Bentson}},
  \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Emma}},\ and\ \bibinfo
  {author} {\bibfnamefont {P.}~\bibnamefont {Krejcik}},\ }\bibfield  {title}
  {\bibinfo {title} {{A transverse rf deflecting structure for bunch length and
  phase space diagnostics}},\ }in\ \href
  {https://doi.org/10.1109/PAC.2001.987379} {\emph {\bibinfo {booktitle}
  {{PACS2001. Proceedings of the 2001 Particle Accelerator Conference (Cat.
  No.01CH37268)}}}}\ (\bibinfo  {publisher} {IEEE},\ \bibinfo {year} {2001})\
  pp.\ \bibinfo {pages} {2353--2355}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Behrens}\ \emph {et~al.}(2014)\citenamefont
  {Behrens}, \citenamefont {Decker}, \citenamefont {Ding}, \citenamefont
  {Dolgashev}, \citenamefont {Frisch}, \citenamefont {Huang}, \citenamefont
  {Krejcik}, \citenamefont {Loos}, \citenamefont {Lutman}, \citenamefont
  {Maxwell}, \citenamefont {Turner}, \citenamefont {Wang}, \citenamefont
  {Wang}, \citenamefont {Welch},\ and\ \citenamefont {Wu}}]{Behrens.2014}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.}~\bibnamefont
  {Behrens}}, \bibinfo {author} {\bibfnamefont {F.-J.}\ \bibnamefont {Decker}},
  \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Ding}}, \bibinfo {author}
  {\bibfnamefont {V.~A.}\ \bibnamefont {Dolgashev}}, \bibinfo {author}
  {\bibfnamefont {J.}~\bibnamefont {Frisch}}, \bibinfo {author} {\bibfnamefont
  {Z.}~\bibnamefont {Huang}}, \bibinfo {author} {\bibfnamefont
  {P.}~\bibnamefont {Krejcik}}, \bibinfo {author} {\bibfnamefont
  {H.}~\bibnamefont {Loos}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Lutman}}, \bibinfo {author} {\bibfnamefont {T.~J.}\ \bibnamefont {Maxwell}},
  \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Turner}}, \bibinfo
  {author} {\bibfnamefont {J.}~\bibnamefont {Wang}}, \bibinfo {author}
  {\bibfnamefont {M.-H.}\ \bibnamefont {Wang}}, \bibinfo {author}
  {\bibfnamefont {J.}~\bibnamefont {Welch}},\ and\ \bibinfo {author}
  {\bibfnamefont {J.}~\bibnamefont {Wu}},\ }\bibfield  {title} {\bibinfo
  {title} {{Few-femtosecond time-resolved measurements of X-ray free-electron
  lasers}},\ }\href {https://doi.org/10.1038/ncomms4762} {\bibfield  {journal}
  {\bibinfo  {journal} {Nat. Commun.}\ }\textbf {\bibinfo {volume} {5}},\
  \bibinfo {pages} {3762} (\bibinfo {year} {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Dolgashev}\ \emph {et~al.}(2014)\citenamefont
  {Dolgashev}, \citenamefont {Bowden}, \citenamefont {Ding}, \citenamefont
  {Emma}, \citenamefont {Krejcik}, \citenamefont {Lewandowski}, \citenamefont
  {Limborg}, \citenamefont {Litos}, \citenamefont {Wang},\ and\ \citenamefont
  {Xiang}}]{Dolgashev.2014}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {V.~A.}\ \bibnamefont
  {Dolgashev}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Bowden}},
  \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Ding}}, \bibinfo {author}
  {\bibfnamefont {P.}~\bibnamefont {Emma}}, \bibinfo {author} {\bibfnamefont
  {P.}~\bibnamefont {Krejcik}}, \bibinfo {author} {\bibfnamefont
  {J.}~\bibnamefont {Lewandowski}}, \bibinfo {author} {\bibfnamefont
  {C.}~\bibnamefont {Limborg}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Litos}}, \bibinfo {author} {\bibfnamefont
  {J.}~\bibnamefont {Wang}},\ and\ \bibinfo {author} {\bibfnamefont
  {D.}~\bibnamefont {Xiang}},\ }\bibfield  {title} {\bibinfo {title} {{Design
  and application of multimegawatt X -band deflectors for femtosecond electron
  beam diagnostics}},\ }\href {https://doi.org/10.1103/PhysRevSTAB.17.102801}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Spec. Top. Accel
  Beams}\ }\textbf {\bibinfo {volume} {17}},\ \bibinfo {pages} {102801}
  (\bibinfo {year} {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Floettmann}\ and\ \citenamefont
  {Paramonov}(2014)}]{Floettmann.2014}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {K.}~\bibnamefont
  {Floettmann}}\ and\ \bibinfo {author} {\bibfnamefont {V.~V.}\ \bibnamefont
  {Paramonov}},\ }\bibfield  {title} {\bibinfo {title} {{Beam dynamics in
  transverse deflecting rf structures}},\ }\href
  {https://doi.org/10.1103/PhysRevSTAB.17.024001} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Spec. Top. Accel Beams}\ }\textbf {\bibinfo
  {volume} {17}},\ \bibinfo {pages} {024001} (\bibinfo {year}
  {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Maxson}\ \emph {et~al.}(2017)\citenamefont {Maxson},
  \citenamefont {Cesar}, \citenamefont {Calmasini}, \citenamefont {Ody},
  \citenamefont {Musumeci},\ and\ \citenamefont {Alesini}}]{Maxson.2017}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Maxson}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Cesar}},
  \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Calmasini}}, \bibinfo
  {author} {\bibfnamefont {A.}~\bibnamefont {Ody}}, \bibinfo {author}
  {\bibfnamefont {P.}~\bibnamefont {Musumeci}},\ and\ \bibinfo {author}
  {\bibfnamefont {D.}~\bibnamefont {Alesini}},\ }\bibfield  {title} {\bibinfo
  {title} {{Direct Measurement of Sub-10 fs Relativistic Electron Beams with
  Ultralow Emittance}},\ }\href
  {https://doi.org/10.1103/PhysRevLett.118.154802} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {118}},\
  \bibinfo {pages} {154802} (\bibinfo {year} {2017})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Tan}\ \emph {et~al.}(2019)\citenamefont {Tan},
  \citenamefont {Fang}, \citenamefont {Tong}, \citenamefont {Gu}, \citenamefont
  {Huang}, \citenamefont {Li}, \citenamefont {Higo}, \citenamefont {Matsumoto},
  \citenamefont {Takatomi},\ and\ \citenamefont {Zhao}}]{Tan.2019}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Tan}}, \bibinfo {author} {\bibfnamefont {W.}~\bibnamefont {Fang}}, \bibinfo
  {author} {\bibfnamefont {D.}~\bibnamefont {Tong}}, \bibinfo {author}
  {\bibfnamefont {Q.}~\bibnamefont {Gu}}, \bibinfo {author} {\bibfnamefont
  {X.}~\bibnamefont {Huang}}, \bibinfo {author} {\bibfnamefont
  {Z.}~\bibnamefont {Li}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont
  {Higo}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Matsumoto}},
  \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Takatomi}},\ and\
  \bibinfo {author} {\bibfnamefont {Z.}~\bibnamefont {Zhao}},\ }\bibfield
  {title} {\bibinfo {title} {{Design, RF measurement, tuning, and high-power
  test of an X-band deflector for Soft X-ray Free Electron Lasers (SXFEL) at
  SINAP}},\ }\href {https://doi.org/10.1016/j.nima.2019.03.093} {\bibfield
  {journal} {\bibinfo  {journal} {Nucl. Instrum. Methods Phys. Res., Sect. A}\
  }\textbf {\bibinfo {volume} {930}},\ \bibinfo {pages} {210} (\bibinfo {year}
  {2019})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Marchetti}\ \emph {et~al.}(2021)\citenamefont
  {Marchetti}, \citenamefont {Grudiev}, \citenamefont {Craievich},
  \citenamefont {Assmann}, \citenamefont {Braun}, \citenamefont {{Catalan
  Lasheras}}, \citenamefont {Christie}, \citenamefont {D'Arcy}, \citenamefont
  {Fortunati}, \citenamefont {Ganter}, \citenamefont {{Gonz{\'a}lez Caminal}},
  \citenamefont {Hoffmann}, \citenamefont {Huening}, \citenamefont
  {Jaster-Merz}, \citenamefont {Jonas}, \citenamefont {Marcellini},
  \citenamefont {Marx}, \citenamefont {McMonagle}, \citenamefont {Osterhoff},
  \citenamefont {Pedrozzi}, \citenamefont {{Prat Costa}}, \citenamefont
  {Reiche}, \citenamefont {Reukauff}, \citenamefont {Schreiber}, \citenamefont
  {Tews}, \citenamefont {Vogt}, \citenamefont {Wesch},\ and\ \citenamefont
  {Wuensch}}]{Marchetti.2021}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Marchetti}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Grudiev}},
  \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Craievich}}, \bibinfo
  {author} {\bibfnamefont {R.}~\bibnamefont {Assmann}}, \bibinfo {author}
  {\bibfnamefont {H.-H.}\ \bibnamefont {Braun}}, \bibinfo {author}
  {\bibfnamefont {N.}~\bibnamefont {{Catalan Lasheras}}}, \bibinfo {author}
  {\bibfnamefont {F.}~\bibnamefont {Christie}}, \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {D'Arcy}}, \bibinfo {author} {\bibfnamefont
  {R.}~\bibnamefont {Fortunati}}, \bibinfo {author} {\bibfnamefont
  {R.}~\bibnamefont {Ganter}}, \bibinfo {author} {\bibfnamefont
  {P.}~\bibnamefont {{Gonz{\'a}lez Caminal}}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Hoffmann}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Huening}}, \bibinfo {author} {\bibfnamefont {S.~M.}\
  \bibnamefont {Jaster-Merz}}, \bibinfo {author} {\bibfnamefont
  {R.}~\bibnamefont {Jonas}}, \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Marcellini}}, \bibinfo {author} {\bibfnamefont
  {D.}~\bibnamefont {Marx}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {McMonagle}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Osterhoff}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Pedrozzi}},
  \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {{Prat Costa}}}, \bibinfo
  {author} {\bibfnamefont {S.}~\bibnamefont {Reiche}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Reukauff}}, \bibinfo {author}
  {\bibfnamefont {S.}~\bibnamefont {Schreiber}}, \bibinfo {author}
  {\bibfnamefont {G.}~\bibnamefont {Tews}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Vogt}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Wesch}},\ and\ \bibinfo {author} {\bibfnamefont {W.}~\bibnamefont
  {Wuensch}},\ }\bibfield  {title} {\bibinfo {title} {{Experimental
  demonstration of novel beam characterization using a polarizable X-band
  transverse deflection structure}},\ }\href
  {https://doi.org/10.1038/s41598-021-82687-2} {\bibfield  {journal} {\bibinfo
  {journal} {Sci. Rep.}\ }\textbf {\bibinfo {volume} {11}},\ \bibinfo {pages}
  {3560} (\bibinfo {year} {2021})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Prat}\ and\ \citenamefont {Aiba}(2014)}]{Prat.2014}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Prat}}\ and\ \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Aiba}},\
  }\bibfield  {title} {\bibinfo {title} {{Four-dimensional transverse beam
  matrix measurement using the multiple-quadrupole scan technique}},\ }\href
  {https://doi.org/10.1103/PhysRevSTAB.17.052801} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Spec. Top. Accel Beams}\ }\textbf {\bibinfo
  {volume} {17}},\ \bibinfo {pages} {052801} (\bibinfo {year}
  {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ji}\ \emph {et~al.}(2019)\citenamefont {Ji},
  \citenamefont {Navarro}, \citenamefont {Musumeci}, \citenamefont {Durham},
  \citenamefont {Minor},\ and\ \citenamefont {Filippetto}}]{Ji.2019}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Ji}}, \bibinfo {author} {\bibfnamefont {J.~G.}\ \bibnamefont {Navarro}},
  \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Musumeci}}, \bibinfo
  {author} {\bibfnamefont {D.~B.}\ \bibnamefont {Durham}}, \bibinfo {author}
  {\bibfnamefont {A.~M.}\ \bibnamefont {Minor}},\ and\ \bibinfo {author}
  {\bibfnamefont {D.}~\bibnamefont {Filippetto}},\ }\bibfield  {title}
  {\bibinfo {title} {{Knife-edge based measurement of the 4D transverse phase
  space of electron beams with picometer-scale emittance}},\ }\href
  {https://doi.org/10.1103/PhysRevAccelBeams.22.082801} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Accel. Beams}\ }\textbf {\bibinfo {volume}
  {22}},\ \bibinfo {pages} {082801} (\bibinfo {year} {2019})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Fritzler}\ \emph {et~al.}(2004)\citenamefont
  {Fritzler}, \citenamefont {Lefebvre}, \citenamefont {Malka}, \citenamefont
  {Burgy}, \citenamefont {Dangor}, \citenamefont {Krushelnick}, \citenamefont
  {Mangles}, \citenamefont {Najmudin}, \citenamefont {Rousseau},\ and\
  \citenamefont {Walton}}]{Fritzler.2004}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Fritzler}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Lefebvre}},
  \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Malka}}, \bibinfo
  {author} {\bibfnamefont {F.}~\bibnamefont {Burgy}}, \bibinfo {author}
  {\bibfnamefont {A.~E.}\ \bibnamefont {Dangor}}, \bibinfo {author}
  {\bibfnamefont {K.}~\bibnamefont {Krushelnick}}, \bibinfo {author}
  {\bibfnamefont {S.~P.~D.}\ \bibnamefont {Mangles}}, \bibinfo {author}
  {\bibfnamefont {Z.}~\bibnamefont {Najmudin}}, \bibinfo {author}
  {\bibfnamefont {J.-P.}\ \bibnamefont {Rousseau}},\ and\ \bibinfo {author}
  {\bibfnamefont {B.}~\bibnamefont {Walton}},\ }\bibfield  {title} {\bibinfo
  {title} {{Emittance measurements of a laser-wakefield-accelerated electron
  beam}},\ }\href {https://doi.org/10.1103/PhysRevLett.92.165006} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {92}},\ \bibinfo {pages} {165006} (\bibinfo {year}
  {2004})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Shanks}\ \emph {et~al.}(2009)\citenamefont {Shanks},
  \citenamefont {Anania}, \citenamefont {Brunetti}, \citenamefont {Cipiccia},
  \citenamefont {Ersfeld}, \citenamefont {Gallacher}, \citenamefont {Issac},
  \citenamefont {Islam}, \citenamefont {Vieux}, \citenamefont {Welsh},
  \citenamefont {Wiggins},\ and\ \citenamefont {Jaroszynski}}]{Shanks.2009}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R.~P.}\ \bibnamefont
  {Shanks}}, \bibinfo {author} {\bibfnamefont {M.~P.}\ \bibnamefont {Anania}},
  \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Brunetti}}, \bibinfo
  {author} {\bibfnamefont {S.}~\bibnamefont {Cipiccia}}, \bibinfo {author}
  {\bibfnamefont {B.}~\bibnamefont {Ersfeld}}, \bibinfo {author} {\bibfnamefont
  {J.~G.}\ \bibnamefont {Gallacher}}, \bibinfo {author} {\bibfnamefont {R.~C.}\
  \bibnamefont {Issac}}, \bibinfo {author} {\bibfnamefont {M.~R.}\ \bibnamefont
  {Islam}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Vieux}},
  \bibinfo {author} {\bibfnamefont {G.~H.}\ \bibnamefont {Welsh}}, \bibinfo
  {author} {\bibfnamefont {S.~M.}\ \bibnamefont {Wiggins}},\ and\ \bibinfo
  {author} {\bibfnamefont {D.~A.}\ \bibnamefont {Jaroszynski}},\ }\bibfield
  {title} {\bibinfo {title} {{Pepper-pot emittance measurement of laser-plasma
  wakefield accelerated electrons}},\ }in\ \href
  {https://doi.org/10.1117/12.820706} {\emph {\bibinfo {booktitle} {{Harnessing
  Relativistic Plasma Waves as Novel Radiation Sources from Terahertz to X-Rays
  and Beyond}}}},\ \bibinfo {series and number} {{SPIE Proceedings}},\ \bibinfo
  {editor} {edited by\ \bibinfo {editor} {\bibfnamefont {D.~A.}\ \bibnamefont
  {Jaroszynski}}\ and\ \bibinfo {editor} {\bibfnamefont {A.}~\bibnamefont
  {Rousse}}}\ (\bibinfo  {publisher} {SPIE},\ \bibinfo {year} {2009})\ p.\
  \bibinfo {pages} {735907}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Sears}\ \emph {et~al.}(2010)\citenamefont {Sears},
  \citenamefont {Buck}, \citenamefont {Schmid}, \citenamefont {Mikhailova},
  \citenamefont {Krausz},\ and\ \citenamefont {Veisz}}]{Sears.2010}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.~M.~S.}\
  \bibnamefont {Sears}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Buck}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Schmid}},
  \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Mikhailova}}, \bibinfo
  {author} {\bibfnamefont {F.}~\bibnamefont {Krausz}},\ and\ \bibinfo {author}
  {\bibfnamefont {L.}~\bibnamefont {Veisz}},\ }\bibfield  {title} {\bibinfo
  {title} {{Emittance and divergence of laser wakefield accelerated
  electrons}},\ }\href {https://doi.org/10.1103/PhysRevSTAB.13.092803}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. ST Accel. Beams}\
  }\textbf {\bibinfo {volume} {13}},\ \bibinfo {pages} {092803} (\bibinfo
  {year} {2010})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Brunetti}\ \emph {et~al.}(2010)\citenamefont
  {Brunetti}, \citenamefont {Shanks}, \citenamefont {Manahan}, \citenamefont
  {Islam}, \citenamefont {Ersfeld}, \citenamefont {Anania}, \citenamefont
  {Cipiccia}, \citenamefont {Issac}, \citenamefont {Raj}, \citenamefont
  {Vieux}, \citenamefont {Welsh}, \citenamefont {Wiggins},\ and\ \citenamefont
  {Jaroszynski}}]{Brunetti.2010}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Brunetti}}, \bibinfo {author} {\bibfnamefont {R.~P.}\ \bibnamefont
  {Shanks}}, \bibinfo {author} {\bibfnamefont {G.~G.}\ \bibnamefont {Manahan}},
  \bibinfo {author} {\bibfnamefont {M.~R.}\ \bibnamefont {Islam}}, \bibinfo
  {author} {\bibfnamefont {B.}~\bibnamefont {Ersfeld}}, \bibinfo {author}
  {\bibfnamefont {M.~P.}\ \bibnamefont {Anania}}, \bibinfo {author}
  {\bibfnamefont {S.}~\bibnamefont {Cipiccia}}, \bibinfo {author}
  {\bibfnamefont {R.~C.}\ \bibnamefont {Issac}}, \bibinfo {author}
  {\bibfnamefont {G.}~\bibnamefont {Raj}}, \bibinfo {author} {\bibfnamefont
  {G.}~\bibnamefont {Vieux}}, \bibinfo {author} {\bibfnamefont {G.~H.}\
  \bibnamefont {Welsh}}, \bibinfo {author} {\bibfnamefont {S.~M.}\ \bibnamefont
  {Wiggins}},\ and\ \bibinfo {author} {\bibfnamefont {D.~A.}\ \bibnamefont
  {Jaroszynski}},\ }\bibfield  {title} {\bibinfo {title} {{Low emittance, high
  brilliance relativistic electron beams from a laser-plasma accelerator}},\
  }\href {https://doi.org/10.1103/PhysRevLett.105.215007} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {105}},\
  \bibinfo {pages} {215007} (\bibinfo {year} {2010})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Manahan}\ \emph {et~al.}(2014)\citenamefont
  {Manahan}, \citenamefont {Brunetti}, \citenamefont {Aniculaesei},
  \citenamefont {Anania}, \citenamefont {Cipiccia}, \citenamefont {Islam},
  \citenamefont {Grant}, \citenamefont {Subiel}, \citenamefont {Shanks},
  \citenamefont {Issac}, \citenamefont {Welsh}, \citenamefont {Wiggins},\ and\
  \citenamefont {Jaroszynski}}]{Manahan.2014}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.~G.}\ \bibnamefont
  {Manahan}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Brunetti}},
  \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Aniculaesei}}, \bibinfo
  {author} {\bibfnamefont {M.~P.}\ \bibnamefont {Anania}}, \bibinfo {author}
  {\bibfnamefont {S.}~\bibnamefont {Cipiccia}}, \bibinfo {author}
  {\bibfnamefont {M.~R.}\ \bibnamefont {Islam}}, \bibinfo {author}
  {\bibfnamefont {D.~W.}\ \bibnamefont {Grant}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Subiel}}, \bibinfo {author} {\bibfnamefont
  {R.~P.}\ \bibnamefont {Shanks}}, \bibinfo {author} {\bibfnamefont {R.~C.}\
  \bibnamefont {Issac}}, \bibinfo {author} {\bibfnamefont {G.~H.}\ \bibnamefont
  {Welsh}}, \bibinfo {author} {\bibfnamefont {S.~M.}\ \bibnamefont {Wiggins}},\
  and\ \bibinfo {author} {\bibfnamefont {D.~A.}\ \bibnamefont {Jaroszynski}},\
  }\bibfield  {title} {\bibinfo {title} {{Characterization of laser-driven
  single and double electron bunches with a permanent magnet quadrupole triplet
  and pepper-pot mask}},\ }\href
  {https://doi.org/10.1088/1367-2630/16/10/103006} {\bibfield  {journal}
  {\bibinfo  {journal} {New J. Phys.}\ }\textbf {\bibinfo {volume} {16}},\
  \bibinfo {pages} {103006} (\bibinfo {year} {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Tenenbaum}\ and\ \citenamefont
  {Shintake}(1999)}]{Tenenbaum.1999}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {P.}~\bibnamefont
  {Tenenbaum}}\ and\ \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont
  {Shintake}},\ }\bibfield  {title} {\bibinfo {title} {{Measurement of small
  electron-beam Spots}},\ }\href
  {https://doi.org/10.1146/annurev.nucl.49.1.125} {\bibfield  {journal}
  {\bibinfo  {journal} {Annu. Rev. Nucl. Part. Sci.}\ }\textbf {\bibinfo
  {volume} {49}},\ \bibinfo {pages} {125} (\bibinfo {year} {1999})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Yan}\ \emph {et~al.}(2012)\citenamefont {Yan},
  \citenamefont {Oroku}, \citenamefont {Yamaguchi}, \citenamefont {Yamanaka},
  \citenamefont {Kamiya}, \citenamefont {Suehara}, \citenamefont {Komamiya},
  \citenamefont {Okugi}, \citenamefont {Terunuma}, \citenamefont {Tauchi},
  \citenamefont {Araki},\ and\ \citenamefont {Urakawa}}]{Yan.2012}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Yan}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Oroku}}, \bibinfo
  {author} {\bibfnamefont {Y.}~\bibnamefont {Yamaguchi}}, \bibinfo {author}
  {\bibfnamefont {T.}~\bibnamefont {Yamanaka}}, \bibinfo {author}
  {\bibfnamefont {Y.}~\bibnamefont {Kamiya}}, \bibinfo {author} {\bibfnamefont
  {T.}~\bibnamefont {Suehara}}, \bibinfo {author} {\bibfnamefont
  {S.}~\bibnamefont {Komamiya}}, \bibinfo {author} {\bibfnamefont
  {T.}~\bibnamefont {Okugi}}, \bibinfo {author} {\bibfnamefont
  {N.}~\bibnamefont {Terunuma}}, \bibinfo {author} {\bibfnamefont
  {T.}~\bibnamefont {Tauchi}}, \bibinfo {author} {\bibfnamefont
  {S.}~\bibnamefont {Araki}},\ and\ \bibinfo {author} {\bibfnamefont
  {J.}~\bibnamefont {Urakawa}},\ }\bibfield  {title} {\bibinfo {title}
  {{Shintake Monitor Nanometer Beam Size Measurement and Beam Tuning}},\ }\href
  {https://doi.org/10.1016/j.phpro.2012.02.522} {\bibfield  {journal} {\bibinfo
   {journal} {Physics Procedia}\ }\textbf {\bibinfo {volume} {37}},\ \bibinfo
  {pages} {1989} (\bibinfo {year} {2012})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Seidel}\ \emph {et~al.}(2021)\citenamefont {Seidel},
  \citenamefont {Osterhoff},\ and\ \citenamefont {Zepf}}]{Seidel.2021}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Seidel}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Osterhoff}},\
  and\ \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Zepf}},\ }\bibfield
  {title} {\bibinfo {title} {{Characterizing ultralow emittance electron beams
  using structured light fields}},\ }\href
  {https://doi.org/10.1103/PhysRevAccelBeams.24.012803} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Accel. Beams}\ }\textbf {\bibinfo {volume}
  {24}},\ \bibinfo {pages} {012803} (\bibinfo {year} {2021})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Antici}\ \emph {et~al.}(2012)\citenamefont {Antici},
  \citenamefont {Bacci}, \citenamefont {Benedetti}, \citenamefont {Chiadroni},
  \citenamefont {Ferrario}, \citenamefont {Rossi}, \citenamefont {Lancia},
  \citenamefont {Migliorati}, \citenamefont {Mostacci}, \citenamefont
  {Palumbo},\ and\ \citenamefont {Serafini}}]{Antici.2012}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {P.}~\bibnamefont
  {Antici}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Bacci}},
  \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Benedetti}}, \bibinfo
  {author} {\bibfnamefont {E.}~\bibnamefont {Chiadroni}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Ferrario}}, \bibinfo {author}
  {\bibfnamefont {A.~R.}\ \bibnamefont {Rossi}}, \bibinfo {author}
  {\bibfnamefont {L.}~\bibnamefont {Lancia}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Migliorati}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Mostacci}}, \bibinfo {author} {\bibfnamefont
  {L.}~\bibnamefont {Palumbo}},\ and\ \bibinfo {author} {\bibfnamefont
  {L.}~\bibnamefont {Serafini}},\ }\bibfield  {title} {\bibinfo {title}
  {{Laser-driven electron beamlines generated by coupling laser-plasma sources
  with conventional transport systems}},\ }\href
  {https://doi.org/10.1063/1.4740456} {\bibfield  {journal} {\bibinfo
  {journal} {J. Appl. Phys.}\ }\textbf {\bibinfo {volume} {112}},\ \bibinfo
  {pages} {044902} (\bibinfo {year} {2012})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Floettmann}(2003)}]{Floettmann.2003}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {K.}~\bibnamefont
  {Floettmann}},\ }\bibfield  {title} {\bibinfo {title} {{Some basic features
  of the beam emittance}},\ }\href
  {https://doi.org/10.1103/PhysRevSTAB.6.034202} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. ST Accel. Beams}\ }\textbf {\bibinfo
  {volume} {6}},\ \bibinfo {pages} {034202} (\bibinfo {year}
  {2003})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Migliorati}\ \emph {et~al.}(2013)\citenamefont
  {Migliorati}, \citenamefont {Bacci}, \citenamefont {Benedetti}, \citenamefont
  {Chiadroni}, \citenamefont {Ferrario}, \citenamefont {Mostacci},
  \citenamefont {Palumbo}, \citenamefont {Rossi}, \citenamefont {Serafini},\
  and\ \citenamefont {Antici}}]{Migliorati.2013}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Migliorati}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Bacci}},
  \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Benedetti}}, \bibinfo
  {author} {\bibfnamefont {E.}~\bibnamefont {Chiadroni}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Ferrario}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Mostacci}}, \bibinfo {author}
  {\bibfnamefont {L.}~\bibnamefont {Palumbo}}, \bibinfo {author} {\bibfnamefont
  {A.~R.}\ \bibnamefont {Rossi}}, \bibinfo {author} {\bibfnamefont
  {L.}~\bibnamefont {Serafini}},\ and\ \bibinfo {author} {\bibfnamefont
  {P.}~\bibnamefont {Antici}},\ }\bibfield  {title} {\bibinfo {title}
  {{Intrinsic normalized emittance growth in laser-driven electron
  accelerators}},\ }\href {https://doi.org/10.1103/PhysRevSTAB.16.011302}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. ST Accel. Beams}\
  }\textbf {\bibinfo {volume} {16}},\ \bibinfo {pages} {011302} (\bibinfo
  {year} {2013})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Humphries}(1990)}]{Humphries.1990}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Humphries}},\ }\href@noop {} {\emph {\bibinfo {title} {{Charged particle
  beams}}}}\ (\bibinfo  {publisher} {{John Wiley and Sons}},\ \bibinfo {year}
  {1990})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Zhang}(1996)}]{Zhang.1996}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Zhang}},\ }\bibfield  {title} {\bibinfo {title} {{Emittance formula for
  slits and pepper-pot measurement}},\ }\bibfield  {journal} {\bibinfo
  {journal} {Fermilab-TM-1988}\ }\href {https://doi.org/10.2172/395453}
  {10.2172/395453} (\bibinfo {year} {1996})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kuschel}\ \emph {et~al.}(2018)\citenamefont
  {Kuschel}, \citenamefont {Schwab}, \citenamefont {Yeung}, \citenamefont
  {Hollatz}, \citenamefont {Seidel}, \citenamefont {Ziegler}, \citenamefont
  {S{\"a}vert}, \citenamefont {Kaluza},\ and\ \citenamefont
  {Zepf}}]{Kuschel.2018}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Kuschel}}, \bibinfo {author} {\bibfnamefont {M.~B.}\ \bibnamefont {Schwab}},
  \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Yeung}}, \bibinfo
  {author} {\bibfnamefont {D.}~\bibnamefont {Hollatz}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Seidel}}, \bibinfo {author} {\bibfnamefont
  {W.}~\bibnamefont {Ziegler}}, \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {S{\"a}vert}}, \bibinfo {author} {\bibfnamefont {M.~C.}\
  \bibnamefont {Kaluza}},\ and\ \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Zepf}},\ }\bibfield  {title} {\bibinfo {title}
  {{Controlling the Self-Injection Threshold in Laser Wakefield
  Accelerators}},\ }\href {https://doi.org/10.1103/PhysRevLett.121.154801}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {121}},\ \bibinfo {pages} {154801} (\bibinfo {year}
  {2018})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {{Oxford
  Instruments}}(2022)}]{OxfordInstruments.2022}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {{Oxford
  Instruments}}},\ }\href
  {https://andor.oxinst.com/products/scmos-camera-series/marana-scmos}
  {\bibinfo {title} {{Marana sCMOS - Andor}}} (\bibinfo {year} {2022}),\
  \bibinfo {note} {accessed: 07. Nov. 2022}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Corde}\ \emph {et~al.}(2011)\citenamefont {Corde},
  \citenamefont {Phuoc}, \citenamefont {Fitour}, \citenamefont {Faure},
  \citenamefont {Tafzi}, \citenamefont {Goddet}, \citenamefont {Malka},\ and\
  \citenamefont {Rousse}}]{Corde.2011}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Corde}}, \bibinfo {author} {\bibfnamefont {K.~T.}\ \bibnamefont {Phuoc}},
  \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Fitour}}, \bibinfo
  {author} {\bibfnamefont {J.}~\bibnamefont {Faure}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Tafzi}}, \bibinfo {author} {\bibfnamefont
  {J.~P.}\ \bibnamefont {Goddet}}, \bibinfo {author} {\bibfnamefont
  {V.}~\bibnamefont {Malka}},\ and\ \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Rousse}},\ }\bibfield  {title} {\bibinfo {title}
  {{Controlled betatron x-ray radiation from tunable optically injected
  electrons}},\ }\href {https://doi.org/10.1103/PhysRevLett.107.255003}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {107}},\ \bibinfo {pages} {255003} (\bibinfo {year}
  {2011})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Schnell}\ \emph {et~al.}(2012)\citenamefont
  {Schnell}, \citenamefont {S{\"a}vert}, \citenamefont {Landgraf},
  \citenamefont {Reuter}, \citenamefont {Nicolai}, \citenamefont {J{\"a}ckel},
  \citenamefont {Peth}, \citenamefont {Thiele}, \citenamefont {Jansen},
  \citenamefont {Pukhov}, \citenamefont {Willi}, \citenamefont {Kaluza},\ and\
  \citenamefont {Spielmann}}]{Schnell.2012}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Schnell}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {S{\"a}vert}},
  \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Landgraf}}, \bibinfo
  {author} {\bibfnamefont {M.}~\bibnamefont {Reuter}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Nicolai}}, \bibinfo {author} {\bibfnamefont
  {O.}~\bibnamefont {J{\"a}ckel}}, \bibinfo {author} {\bibfnamefont
  {C.}~\bibnamefont {Peth}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont
  {Thiele}}, \bibinfo {author} {\bibfnamefont {O.}~\bibnamefont {Jansen}},
  \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Pukhov}}, \bibinfo
  {author} {\bibfnamefont {O.}~\bibnamefont {Willi}}, \bibinfo {author}
  {\bibfnamefont {M.~C.}\ \bibnamefont {Kaluza}},\ and\ \bibinfo {author}
  {\bibfnamefont {C.}~\bibnamefont {Spielmann}},\ }\bibfield  {title} {\bibinfo
  {title} {{Deducing the electron-beam diameter in a laser-plasma accelerator
  using x-ray betatron radiation}},\ }\href
  {https://doi.org/10.1103/PhysRevLett.108.075001} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {108}},\
  \bibinfo {pages} {075001} (\bibinfo {year} {2012})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Plateau}\ \emph {et~al.}(2012)\citenamefont
  {Plateau}, \citenamefont {Geddes}, \citenamefont {Thorn}, \citenamefont
  {Chen}, \citenamefont {Benedetti}, \citenamefont {Esarey}, \citenamefont
  {Gonsalves}, \citenamefont {Matlis}, \citenamefont {Nakamura}, \citenamefont
  {Schroeder}, \citenamefont {Shiraishi}, \citenamefont {Sokollik},
  \citenamefont {{van Tilborg}}, \citenamefont {Toth}, \citenamefont
  {Trotsenko}, \citenamefont {Kim}, \citenamefont {Battaglia}, \citenamefont
  {St{\"o}hlker},\ and\ \citenamefont {Leemans}}]{Plateau.2012}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.~R.}\ \bibnamefont
  {Plateau}}, \bibinfo {author} {\bibfnamefont {C.~G.~R.}\ \bibnamefont
  {Geddes}}, \bibinfo {author} {\bibfnamefont {D.~B.}\ \bibnamefont {Thorn}},
  \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Chen}}, \bibinfo {author}
  {\bibfnamefont {C.}~\bibnamefont {Benedetti}}, \bibinfo {author}
  {\bibfnamefont {E.}~\bibnamefont {Esarey}}, \bibinfo {author} {\bibfnamefont
  {A.~J.}\ \bibnamefont {Gonsalves}}, \bibinfo {author} {\bibfnamefont {N.~H.}\
  \bibnamefont {Matlis}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont
  {Nakamura}}, \bibinfo {author} {\bibfnamefont {C.~B.}\ \bibnamefont
  {Schroeder}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Shiraishi}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Sokollik}},
  \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {{van Tilborg}}}, \bibinfo
  {author} {\bibfnamefont {C.}~\bibnamefont {Toth}}, \bibinfo {author}
  {\bibfnamefont {S.}~\bibnamefont {Trotsenko}}, \bibinfo {author}
  {\bibfnamefont {T.~S.}\ \bibnamefont {Kim}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Battaglia}}, \bibinfo {author} {\bibfnamefont
  {T.}~\bibnamefont {St{\"o}hlker}},\ and\ \bibinfo {author} {\bibfnamefont
  {W.~P.}\ \bibnamefont {Leemans}},\ }\bibfield  {title} {\bibinfo {title}
  {{Low-emittance electron bunches from a laser-plasma accelerator measured
  using single-shot x-ray spectroscopy}},\ }\href
  {https://doi.org/10.1103/PhysRevLett.109.064802} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {109}},\
  \bibinfo {pages} {064802} (\bibinfo {year} {2012})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Salgado~\textit{et al.}}()}]{emittance-paper}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {F.~C.}\ \bibnamefont
  {Salgado~\textit{et al.}}},\ }\bibfield  {title} {\bibinfo {title}
  {Limitations of emittance and source size measurement of laser-accelerated
  electron beams using pepper pot mask method},\ }\bibinfo {note} {\textit{(to
  be published)}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Derouillat}\ \emph {et~al.}(2018)\citenamefont
  {Derouillat}, \citenamefont {Beck}, \citenamefont {P{\'e}rez}, \citenamefont
  {Vinci}, \citenamefont {Chiaramello}, \citenamefont {Grassi}, \citenamefont
  {Fl{\'e}}, \citenamefont {Bouchard}, \citenamefont {Plotnikov}, \citenamefont
  {Aunai}, \citenamefont {Dargent}, \citenamefont {Riconda},\ and\
  \citenamefont {Grech}}]{Derouillat.2018}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Derouillat}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Beck}},
  \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {P{\'e}rez}}, \bibinfo
  {author} {\bibfnamefont {T.}~\bibnamefont {Vinci}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Chiaramello}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Grassi}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Fl{\'e}}}, \bibinfo {author} {\bibfnamefont
  {G.}~\bibnamefont {Bouchard}}, \bibinfo {author} {\bibfnamefont
  {I.}~\bibnamefont {Plotnikov}}, \bibinfo {author} {\bibfnamefont
  {N.}~\bibnamefont {Aunai}}, \bibinfo {author} {\bibfnamefont
  {J.}~\bibnamefont {Dargent}}, \bibinfo {author} {\bibfnamefont
  {C.}~\bibnamefont {Riconda}},\ and\ \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Grech}},\ }\bibfield  {title} {\bibinfo {title} {{Smilei:
  A collaborative, open-source, multi-purpose particle-in-cell code for plasma
  simulation}},\ }\href {https://doi.org/10.1016/j.cpc.2017.09.024} {\bibfield
  {journal} {\bibinfo  {journal} {Comput. Phys. Commun.}\ }\textbf {\bibinfo
  {volume} {222}},\ \bibinfo {pages} {351} (\bibinfo {year}
  {2018})}\BibitemShut {NoStop}%
\end{thebibliography}%

